Beyond the Hype: A Real-World Evaluation of the Impact and Cost of Machine Learning-Based Malware Detection

In this paper, we present a scientific evaluation of four prominent malware detection tools to assist an organization with two primary questions: To what extent do ML-based tools accurately classify previously- and never-before-seen files? Is it worth purchasing a network-level malware detector? To identify weaknesses, we tested each tool against 3,536 total files (2,554 or 72\% malicious, 982 or 28\% benign) of a variety of file types, including hundreds of malicious zero-days, polyglots, and APT-style files, delivered on multiple protocols. We present statistical results on detection time and accuracy, consider complementary analysis (using multiple tools together), and provide two novel applications of the recent cost-benefit evaluation procedure of Iannacone \& Bridges. While the ML-based tools are more effective at detecting zero-day files and executables, the signature-based tool may still be an overall better option. Both network-based tools provide substantial (simulated) savings when paired with either host tool, yet both show poor detection rates on protocols other than HTTP or SMTP. Our results show that all four tools have near-perfect precision but alarmingly low recall, especially on file types other than executables and office files -- 37% of malware tested, including all polyglot files, were undetected. Priorities for researchers and takeaways for end users are given.

==> 34-confirmatory-results.tex <==

\begin{table*}[t]
    \centering
    \caption{Confirmatory malware detection results by file category}
\begin{tabular}{llllllllllllllll}
\toprule
 \textbf{Category } &   \multicolumn{3}{c}{\textbf{Host Sig.}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Host ML}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Static}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Dyn.}} &   \multicolumn{3}{c}{\textbf{All Four Sensors}} \\
(\#mal/\#benign) & Prec. & Recall &    F1 &                Prec. & Recall &   F1 &                Prec. & Recall &   F1 &              Prec. & Recall &   F1 &            Prec. & Recall &   F1 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{APT} (27/0)       &    1.0&  0.667 &    0.8 &                   1.0&   0.63 &  0.773 &                     1.0&  0.296 &  0.457 &                   1.0&  0.556 &  0.714 &                 1.0&  0.296 &  0.457 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (525/200)    &    1.0& 0.0892 &  0.164 &                    0 &      0 &      0 &                     1.0& 0.0431 & 0.0826 &                   1.0& 0.0462 & 0.0882 &                  0 &      0 &      0 \\
\textbf{Office} (600/200) &    1.0&  0.782 &  0.878 &                    0 &      0 &      0 &                     1.0&  0.728 &  0.842 &                   1.0&  0.613 &   0.76 &                  0 &      0 &      0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF }(600/200)    &    1.0&  0.512 &  0.678 &                    0 &      0 &      0 &                     1.0&  0.448 &  0.618 &                   1.0&  0.497 &  0.664 &                  0 &      0 &      0 \\
\textbf{PE32} (600/200)   &    1.0&  0.505 &  0.671 &                   1.0&  0.455 &  0.625 &                     1.0&   0.33 &  0.496 &                   1.0&  0.318 &  0.482 &                 1.0&  0.273 &  0.428 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (582/182)   &    1.0&  0.233 &  0.377 &                   1.0&  0.188 &  0.316 &                     1.0&  0.205 &   0.34 &                   1.0&  0.193 &  0.323 &                 1.0&  0.168 &  0.287 \\
\textbf{Polyglot} (199/0) &     0 &      0 &      0 &                    0 &      0 &      0 &                      0 &      0 &      0 &                    0 &      0 &      0 &                  0 &      0 &      0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &    1.0& 0.0347 & 0.0671 &                   1.0& 0.0347 & 0.0671 &                     1.0& 0.0298 & 0.0578 &                   1.0& 0.0298 & 0.0578 &                 1.0& 0.0273 & 0.0531 \\
\bottomrule
\end{tabular}
    \label{tab:tc2:conf-analysis}
\end{table*}



\subsection{Confirmatory/Corroborating Sensors}
\label{sec:confirmatory}
In addition to understanding how different sensing tools are complementary, it is useful to understand the extent to which they corroborate each other. 
Note that we use the term ``corroborate" and ``confirm" interchangeably. 
In a diverse sensing environment, confirmatory sensors may provide context as to the severity of an event or reliability of a malware detection.  
In terms of cybersecurity architecture, it can also reveal those sensors that duplicate detection capability.  
Table \ref{tab:tc2:conf-analysis} is a confirmatory analysis of various sensing combinations.  
Similar to complementary analysis, confirmatory analysis considers sensor combinations, but it differs in that it evaluates \textit{intersection} rather than the union of their individual detection results. In analyzing the confirmatory results of sensing combinations, it is interesting to note that the Host Signature-Based Sensor combined with any of the ML-based technologies results in poorer detection performance overall.  
This indicates a low degree of intersection between detection using the signature-based methods vs. the ML-based methods. 
In some cases, such as with MS Office and PDF files, for the Host Signature-Based Sensor $\cap$ Network Static Tool  and PDF files for the Host Signature-Based Sensor $\cap$ Network Dynamic tool, the recall value remains close to their comparative values, indicating that these combinations of tools are assessing malware files consistently for those file categories. 
Given the high precision of the evaluated malware detection technologies, it does not add value to consider them in a confirmatory way, given that their detections are complementary. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/confirmatory-filetype-f1-heatmap}
    \caption{Confirmatory $F_{1} Scores$ by File Category}
    \label{fig:tc2:confirmatory-analysis-fscores}
\end{figure}

An interesting result is the consistency between the union and intersection of the network-based malware analyzers; for most categories, drop-off is minimal regardless of whether these tools are considered in a complementary or confirmatory way. Thus, despite the different modes of sensing (static and dynamic malware analysis), these technologies are assessing malware very consistently and are largely a duplication of capability.
Considering precision and recall together, Figure \ref{fig:tc2:confirmatory-analysis-fscores} shows the F1 scores for all pair-wise combinations of sensors and all file categories, when looking at their corroborating detections.  
% As with previous heatmaps and tables, the Host Signature-Based Sensor  is included alone  as a baseline.  
%As noted in the discussion of Table \ref{tab:tc2:conf-analysis}, the combination of Network Static Tool Cortex $\cap$ Juniper JATP had the overall highest F1 Scores, indicating that these two tools have highly similar analytic value. That is, they are assessing files very similarly.




==> beyond-the-hype-3 (2)/01-packages.tex <==
\usepackage[utf8]{inputenc}

% \usepackage[dvipsnames]{xcolor}
\usepackage{xcolor,colortbl}
\usepackage{epstopdf} 
% \usepackage{cite}
\usepackage{verbatim}
\usepackage{pgfplotstable,filecontents}
\pgfplotsset{compat=1.9}% suppress warning
\usepackage{enumitem}
%wrap urls that are too long
% \usepackage{url}
\usepackage{ulem}
\usepackage{breakurl}
\usepackage{breakcites}
\PassOptionsToPackage{hyphens}{url}
\usepackage{hyperref}
\hypersetup{colorlinks=true,urlcolor=blue}
% \urlstyle{same}
% \renewcommand\UrlFont{\color{blue}\rmfamily}

\usepackage{graphicx}
\usepackage{grffile}


%% HIGHLIGHTING
\usepackage{soulutf8} % allows highlighting w/ \hl
\renewcommand\hl[1]{#1} % redefines \hl to do nothing (uncomment to turn highlighting off). 

%% text wrapped figs and tables:
\usepackage{wrapfig}
\usepackage{longtable,tabu}

%% for nice tables: 
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}% For formal tables
\usepackage{threeparttable}

\usepackage{caption}
\usepackage{subcaption}
\captionsetup{font=small} %% makes captions not look like part of the paper's prose and saves space
% \captionsetup[sub]{font=footnotesize}
\captionsetup[sub]{font=small}
\setlength{\abovecaptionskip}{1pt}
\setlength{\belowcaptionskip}{1.5pt}


\usepackage{rotating}
\usepackage{lipsum}
% \usepackage[toc,page,header]{appendix}

\usepackage{amsmath, breqn}
\newcommand{\smalltilde}{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}} 

\usepackage{fancyhdr}

\newenvironment{ncr}{\par\color{green}}{\par}


\setdescription{topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt, leftmargin=.15cm}


% \usepackage{geometry} %% just including this ruins the margins for lncs

%% used for changing margins to fit the big table: 
\usepackage{changepage}

% \usepackage{etoolbox}
% \patchcmd{\thebibliography}{\chapter*}{\section*}{}{}



%% next two for landscaping tables: 
% \usepackage{geometry}
% \usepackage{pdflscape}

==> beyond-the-hype-3 (2)/02-top.tex <==

\setcopyright{acmcopyright}
\copyrightyear{2022}
\acmYear{2022}
\acmDOI{XXXXXXX.XXXXXXX}

%%
%% These commands are for a JOURNAL article.
\acmJournal{DTRAP}
\acmVolume{00}
\acmNumber{00}
\acmArticle{000}
\acmMonth{1}
%%\acmSubmissionID{123-A56-BU3}

%% Uncommenting the next command will enable different citation style
%%\citestyle{acmauthoryear}


\title[Beyond the Hype]{Beyond the Hype: An Evaluation of Commercially Available Machine-Learning-Based Malware Detectors}
\thanks{\hl{Code for cost model}: %URL REDACTED FOR DOUBLE BLIND REVIEW} 
\url{https://github.com/bridgesra/beyond-the-hype-paper-code}}

% \thanks{\small{This manuscript has been co-authored by UT-Battelle, LLC, under contract DE-AC05-00OR22725 with the US Department of Energy (DOE). The US government retains and the publisher, by accepting the article for publication, acknowledges that the US government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this manuscript, or allow others to do so, for US government purposes. DOE will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (\url{http://energy.gov/downloads/doe-public-access-plan}).}}

% \author{author names redacted}
% \email{email redacted} 
% \affiliation{
%     \institution{affiliations redacted}
%     \country{affiliation redacted}
%     }


\author{Robert~A.~Bridges}
% \authornote{Corresponding author}
% \authornotemark[1]
\orcid{0001-7962-6329}
\email{bridgesra@ornl.gov} 

\author{Sean~Oesch}
\email{oeschts@ornl.gov} 

\author{Michael~D.~Iannacone}
\email{iannaconeme@ornl.gov} 

\author{Kelly~M.~T.~Huffer}
\email{hufferkm@ornl.gov} 

\author{Brian~Jewell}
\email{jewellbc@ornl.gov} 

\author{Jeff~A.~Nichols}
\email{nicholsja@ornl.gov}

\author{Brian~Weber}%\authornotemark[1]
\email{weberb@ornl.gov}
\affiliation{%
    \institution{Oak Ridge National Laboratory}
    \city{Oak Ridge} 
    \state{TN}
    \country{USA}
    }

\author{Miki~E.~Verma}
\email{meverma@stanford.edu} 
\affiliation{%
    \institution{Stanford University}
    \city{Palo Alto} 
    \state{CA}
    \country{USA}
}


\author{Daniel~Scofield}%\authornotemark[2]
% \email{}
\author{Craig~Miles}
% \email{}
\affiliation{
    \institution{Amazon Inc.}
    \country{USA}
}


\author{Thomas~Plummer}
\email{thomas.plummer@lmco.com}
\author{Mark~Daniell}
\email{mark.a.daniell@lmco.com}
\affiliation{
    \institution{Lockheed Martin}
    \country{USA}
}

\author{Anne~M.~Tall}
\email{annetall@mitre.org}
\affiliation{
    \institution{MITRE Corporation}
    \country{USA}
}

\author{Justin M. Beaver} 
\email{jbeaver@lirio.com}
\affiliation{
    \institution{Lirio LLC}
    \country{USA}
}


\author{Jared~M.~Smith}
\email{jaredsmith@securityscorecard.io}
\affiliation{
    \institution{Security Scorecard}
    \country{USA}
    }


%Short authors for page headers: 
\renewcommand{\shortauthors}{Bridges, et al.}


==> beyond-the-hype-3 (2)/04-abstract.tex <==
\begin{abstract}
There is a lack of scientific testing of commercially available malware detectors, especially those that boast accurate classification of never-before-seen (i.e., zero-day) files using machine learning (ML). 
Consequently, efficacy of malware detectors is opaque, inhibiting end users from making informed decisions and researchers from targeting gaps in current detectors. 
In this paper, we present a scientific evaluation of four \hl{prominent commercial} malware detection tools to assist an organization with two primary questions:  
To what extent do ML-based tools accurately classify previously and never-before-seen files? 
\hl{Is purchasing a network-level malware detector worth the cost?} 
To investigate, we tested each tool against 3,536 total files (2,554 or 72\% malicious, 982 or 28\% benign) of a variety of file types, including hundreds of malicious zero-days, polyglots, and APT-style files, delivered on multiple protocols.
We present statistical results on detection time and accuracy, consider complementary analysis (using multiple tools together), and provide two novel applications of the recent cost-benefit evaluation procedure of Iannacone \& Bridges. 
Although the ML-based tools are more effective at detecting zero-day files and executables, the signature-based tool might still be an overall better option. 
Both network-based tools provide substantial (simulated) savings when paired with either host tool, yet both show poor detection rates on protocols other than HTTP or SMTP. 
Our results show that all four tools have near-perfect precision but alarmingly low recall, especially on file types other than executables and office files---37\% of malware, including all polyglot files, were undetected. 
Priorities for researchers and takeaways for end users are given. 
\hl{Code for future use of the cost model is provided.} 
\end{abstract}


==> beyond-the-hype-3 (2)/06-bottom.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002978.10002997.10002998</concept_id>
       <concept_desc>Security and privacy~Malware and its mitigation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978.10003029.10003031</concept_id>
       <concept_desc>Security and privacy~Economics of security and privacy</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Malware and its mitigation}
\ccsdesc[500]{Security and privacy~Economics of security and privacy}

\keywords{malware detection, endpoint detection, network detection, evaluation, test, intrusion detection, cost benefit analysis, static analysis, dynamic analysis, machine learning}

%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\settopmatter{printfolios=true}
\pagenumbering{arabic}

\thanks{\hl{redacted organizational disclaimer}}
% \thanks{This manuscript has been co-authored by UT-Battelle LLC under Contract No. DE-AC05-00OR22725 with the US Department of Energy (DOE). The US government retains and the publisher, by accepting the article for publication, acknowledges that the US government retains a nonexclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this manuscript, or allow others to do so, for US government purposes. DOE will provide public access to these results of federally sponsored research in accordance with the DOE Public Access Plan (\url{http://energy.gov/downloads/doe-public-access-plan}).}


==> beyond-the-hype-3 (2)/10-intro.tex <==


\section{Introduction} 
\label{sec:intro}
Attackers use malicious software, known as \textit{malware}, to steal sensitive data, damage network infrastructure, and hold information for ransom. 
One of the top priorities for computer security tools is to detect malware and prevent or minimize its impact on both corporate and personal networks. %ARTICLE OR CITATION
Traditionally, signature-based methods have been used to detect files previously identified as malicious with near perfect precision, but potentially miss newer malware samples.
With the advent of self-modifying malware and the rapid increase in novel threats, signature-based methods are insufficient on their own. 
By generalizing patterns of known benign/malicious training examples, machine learning (ML) exhibits the capability to quickly and accurately classify novel file samples in many research studies \cite{Gibert_Mateu_Planes_2020}. 
Moreover, ML-based malware research has made the transition from the 
\begin{wrapfigure}[]{r}{.45\textwidth}
    % \vspace{-.4cm}
    % \hspace{-.5cm}
    \centering
    \includegraphics[width=.45\textwidth]{fig/experiment-diagram.eps}
    % \includegraphics[scale=0.33, natwidth=640, natheight=480]{fig/experiment-diagram.png}
    \caption{Malware detection experiment}
    \label{fig:experiment-diagram}
\end{wrapfigure}
subject of myriad research efforts to a current mainstay of commercial-off-the-shelf (COTS) malware detectors. 
Yet, few practical evaluations of COTS ML-based technologies have been conducted. 

\indent\rule{0pt}{0pt}\hl{
Turning from the academic literature to market reports from commercial companies can provide (for a fee) useful information, specifically, end-user feedback, itemization of all technologies in the antivirus/endpoint detection and response marketplace {\cite{gartner-edr}}, and  even statistics showing the efficacy of the detectors on malware tests {\cite{av-test, selabs-test}}. 
(See Related Works {\ref{sec:market-reports}} for recent examples by AV-TEST and SE Labs.) 
Yet, these tests often report near perfect detection for many tools, diminishing trust in the capability of the test to sufficiently stress test the tools or to differentiate the tools.
Further, as our results---under 60\% recall of all tools tested---and other previous works {\cite{christodorescu2004testing}} confirm, these near perfect evaluations promote a false narrative that modern (especially ML-driven) malware detectors provide just shy of perfect protection. 
Even when armed with many statistics on detection capabilities, balancing or weighing these heterogeneous measurements when reasoning about the efficacy of tools is difficult {\cite{iannacone2020quantifiable}}. 
}


As a result, organizations have limited insight into whether or how COTS malware detection tools add value to their current defense solutions, short of trusting possibly skewed vendor-provided claims and market/consumer reports. 
The origin of this paper is evidence of this fact, as the authors were tasked with evaluating four market-leading  malware detection tools to assist in understanding their efficacy. 
This work describes a scientific experiment designed and conducted by the authors (professional researchers) to assist an organization in examining the benefits and tradeoffs of  commercially available ML-based malware detection tools. 


\hl{
Guided by the organization's requests, we established meetings with 22 sales and technical representatives of many popular vendors to learn the merits and approaches of their detection technologies. 
Based on the organization's requirements, four prominent detectors were chosen for study: two host-based (one signature-based, one ML-based) and two network-based (both ML-based, one static, and one dynamic) detectors. 
Of particular interest in this study are 
detection capability across varying file types and categories; 
efficacy of  the network-level detectors across varying protocols; and 
studying value provided by ML- vs. signature-based, host vs. network, and static vs. dynamic tools, with an eye towards ``defense-in-depth,'' (i.e.,  strategically combining tools).  
}
Our overall goal is to provide the funding organization with methods for quantitatively reasoning about malware detectors and to exhibit results on these four tools that can provide insights into two questions: 
% Specific questions of interest included the following:\\ 

\textbf{(Q1) ML Generalization Hypothesis:} We are interested in the fundamental promise of the three ML-based malware detectors; namely,  % (and shedding the memory-intensive libraries of signatures), 
``Can ML-based COTS tools accurately classify both never-before-seen files (especially zero-day malware) and publicly available files?''

\textbf{(Q2) Network-Level Malware Detection Hypothesis:} Network-level malware detectors seek to complement host detectors. They leverage the advantage of greater computational resources (available in a network appliance, generally a commodity server) without affecting users' workstations. 
\hl{ This means, in theory, they can afford more in-depth analysis without impacting usability, namely slowing processes on each workstation.
Notably, the network-level detector must carve the file out of the packets to correctly process it, which is not necessary for host detectors.} 
Of course, if the network detector cannot expand the detection capabilities, it simply adds cost without enhancing defenses. 
In our experience with approximately ten security operation centers (SOCs) 
\cite{oesch2020assessment, bridges2018how},
% \textcolor{red}{[citations redacted]}, 
all centers required endpoint malware detection and signature-based network intrusion detection, but none used network-level malware detection technologies. 
Thus, we investigate the question, ``Is it worth purchasing, configuring, and maintaining a network-level malware detector, given in-place host-based detection?''
%provide quantitative analysis of network-level detectors as complements to endpoint detectors---simply 



% \textbf{Static vs. Dynamic Analysis:} Finally, we wish to again quantify with data the trade-off between detection time and detection accuracy for commercially available static vs. dynamic tools. 


%% how did we do it? 
We were given licenses from four vendors for experimentation under the agreement that results could only be released with anonymity; we are unable to provide any details that might disclose the vendors or their intellectual property. 
The four COTS tools used in this experiment---two endpoint detection tools, one signature based and one claiming to be solely ML based (supervised learning with no signatures), and two network-level tools, both ML based with one claiming static analysis (does not execute files) and the other claiming dynamic analysis (executes files in a sandbox)---provide representatives of different available malware detection approaches.  
The first endpoint malware detector being solely signature based is considered a baseline to represent the status quo for modern commercial malware defenses.  
% The second endpoint malware detection tool claims to use no signatures, relying only on supervised learning techniques. 
% This tool was chosen to allow comparison across the signature vs. the ML dichotomy of endpoint detection products currently available.  
Both network detection tools perform file extraction from packets (whereas endpoint detectors scan files on each host), and both claim to use ML techniques to detect files. 
The first tool uses static analysis and an ensemble of ML- and signature-based detectors.  
The second  tool performs dynamic analysis to feed an ML classifier.
See Section \ref{sec:tools}. 
\hl{We note that two types of commercially available malware detectors are not represented in this study:  those that leverage a cloud connection for interactive intelligence (which can be at the host and/or network level) and network-level detectors that are solely signature based. }


To test these technologies, we configured a network at the National Cyber Range (NCR) \cite{ferguson2014ncr} (see Section \ref{sec:experiment}) to deliver 2,554 malware and 982 benignware samples of varying file types to hosts.  
Zero-days (specially crafted malware never seen in the wild), files to mimic advanced persistent threat (APT) actions, and polyglots (files functioning with multiple file types) were also included to test the capability of these tools to identify novel threats (see Figure \ref{fig:experiment-diagram}).

Statistical results (Section \ref{sec:stats-results}) from the experiment give enlightening insight into how well or how poorly commercially available malware detectors perform. 
Analysis of detection statistics by file type and delivery protocol illuminates rather alarming gaps. 
Comparison of the signature-based tools to the three ML tools, especially on zero-day files, allows us to quantify question (Q1), the ML generalization hypothesis. 
Furthermore, we provide an analysis of conviction latency (i.e., time to detect) per tool and per file type to illustrate the gains/losses of network tools and of using static versus dynamic analysis. 
Under the assumption that host-based malware detection is a requirement,  we consider a defense-in-depth question, ``Is it worthwhile to use multiple detectors together?,'' by simulating complementary detectors using the logical \texttt{OR} of their alerts.   

While these statistical results are enlightening, they present tradeoffs that are difficult to reconcile when choosing the ``best'' malware detection tools (e.g.,  how to balance give and take among detection rates, false alerts, detection delays, and anticipated attack costs). 
% In addition to the usual statistical metrics of detection accuracy, we tailor the new cost--benefit evaluation method of 
To aid the funding organization in using all the results to assess the tools, we design a novel instantiating of  the general cost-benefit framework of Iannacone \& Bridges \cite{iannacone2020quantifiable} to quantifiably assess and compare the network-level tools (question Q(2)). 
This method simulates the cost to an enterprise using the technologies by integrating detection accuracy and time-to-detect statistics (all learned from experimental testing), along with estimates of attack damage costs, labor costs, and resource costs. 
% gauges efficacy by considering how an SOC would use the tool, estimating labor and resource costs for initial and ongoing configuration, triage, incident response, and estimated attack costs. 
% The method takes into account accuracy metrics, time to detection, and expense for purchasing necessary hardware and software licences. 
We configure the cost model to estimate costs of the two network-level tools on the emulated network. Then in a separate evaluation, we estimate the additional costs for adding the network tools to complement each endpoint tool.
Our configuration of the cost model, in particular in evaluating complementary detectors used in tandem, is novel. 
It gives new vantage points for understanding the tools' efficacy  use and provides a procedure to assist future acquisition decisions. 
See Section \ref{sec:cost-model}. 


% a reconfiguration of the cost model to estimate the cost/savings of purchasing each network tool under the (two separate) assumptions that each endpoint tool is and will remain on each host, answering the question ``Given my current endpoint protection, is it worth it to buy one of these network detection tools, and if so, which one saves the most?" 


\subsection{Results Summary}
\hl{The key findings from our experiment are as follows: }
\begin{itemize} 
\item These COTS detectors have nearly perfect precision but with detection rates in the 34--55\% range. 
\item Detection rates jump to $\smalltilde60\%$ for any pair of a host and a network detector; combining more than three detectors does not provide much more gain.
\item From a cost simulation analysis, the host signature-based detector is the best under our baseline assumptions. 
\item When assuming that ``hard'' malware (i.e., zero-days, polyglots, APT-style) files will incur larger damage costs than $n-$day files, ML-based detectors provide greater savings according to our cost model. 
\item Substantial savings are provided when adding one of the network-based detectors, with the dynamic detector providing the largest savings (for both host detectors).
\end{itemize} 



We conclude this paper with a discussion in Section \ref{sec:did-discussion} of the overall takeaways and the limitations of this work. 
These findings are mapped to takeaways for (1) researchers wanting to strengthen the state of malware defense and (2) SOCs considering the purchase of a malware detector. 



\subsection{Contributions} 
% This work makes the following contributions: 
\hl{Our research is one of the few academic studies providing  empirical evaluation of commercially available ML-based malware detection tools, and we believe it is the largest academic evaluation of such tools to date---using a corpus of more than 3,500 files (in comparison to 1,000 files in prior work on COTS {\cite{fleshman2018static}}).}
\hl{More notably, it provides a unique set of files with a wide variety of file types of varying difficulty to detect, illuminating strengths and weaknesses of the tools.  It is in response to commercial evaluations} {\cite{av-test, selabs-test}} \hl{that do provide results of COTS malware detectors on larger corpora but fail to differentiate among the tools.}
\hl{Our contribution is also in our analysis of the results, considering complementary detectors and multiple applications of a cost-benefit analysis.}
% We are the first to quantify the benefits of ML-based vs. signature-based tools, host- vs. network-level detection, and static vs. dynamic analysis using commercially available tools.
We provide two novel contributions to the general cost model framework of Iannacone \& Bridges \cite{iannacone2020quantifiable}. 
We show how to use a large number of benign/malware samples to gain accuracy in detection accuracy statistics, which are needed inputs to the model, while scaling the model to represent a realistic benign/malware ratio in cost calculations. 
Our second configuration of the cost model estimates the additional cost/savings of a network-level tool, which is different and potentially more appropriate or useful than originally proposed. 
\hl{Code for our cost model configuration is provided, see footnote on first page.} 
% We expect this to provide a blueprint for similar future evaluations that can be tailored to a specific SOCs needs. 

Our statistical results provide empirical verification that contributes to a better understanding of the state of commercial malware detection in practice, a problem that has received little attention by researchers; 
in particular, we find several key weaknesses in the four tools investigated, including surprisingly low detection rates (but high precision),  a complete failure to detect polyglot files, and varying detection capabilities across file categories and, for network-level tools, across protocols. 
This helps confirm (at least our, i.e., the authors') suspicions about efficacy of commercial detectors.   
Finally, we map our findings to takeaways first for researchers, giving prioritized research directions to enhance detection in practice, and second for SOC personnel, giving guidance to consider when purchasing such tools. See the discussion in Section \ref{sec:did-discussion}. 
% Overall, this is the first use of the cost model developed by Iannacone and Bridges \cite{iannacone2020quantifiable} to incorporate all measured values into a single quantifiable metric that enables SOCs to make better purchasing decisions. 
% Finally, we map our experimental results to actionable advice for choosing malware detection tools (Section \ref{sec:advice}).




==> beyond-the-hype-3 (2)/12-related-works.tex <==
\section{Related Work}
A large body of work proposes and tests ML algorithms for malware detection, and surveys have collected and organized these works. 
However, to our knowledge,  few works seek to evaluate commercial, especially, ML-based malware detection, and none provides cost-benefit analysis informed by tool-specific detection statistics learned from experimental results for reasoning about these detectors. 
In addition, the most thorough existing evaluation of malware detection tools in the literature uses a corpus of  1,000 samples, compared with our evaluation of more than 3,500 samples. 
Finally, no previous work has the efficacy of pairing complementary detectors as suggested by the ``defense-in-depth'' idea. 
Here we address commercial evaluations, which are much larger than ours, but do not provide differentiation of tools---many tools get near perfect results---inducing skepticism of the efficacy of these evaluations. 

\subsubsection{COTS Evaluations}
Early work by Christodorescu \& Jha \cite{christodorescu2004testing} presents an evaluation of three COTS malware detectors on eight malware, with a goal of studying what signatures a blackhat hacker can learn about a blackbox detector. 
Notably, these authors summarize findings by exclaiming ``From
our experimental results we conclude that the state of the art for malware detectors is dismal!''
The two studies that focus specifically on the capability of existing tools to detect malware use a corpus of 200 samples (100 malicious and 100 benign)~\cite{aslan2017investigation} and 29 samples (all malicious)~\cite{pandey2014performance}, respectively.
The more thorough of these evaluations, conducted by Aslan and Samet~\cite{aslan2017investigation}, finds that static and dynamic analyses work better in tandem than either one on its own and that, in general, dynamic analysis outperforms static. 
Neither of these works focus on the benefit that ML provides for malware detection. 

A large body of work has emerged to evaluate whether adversarial machine learning (AML)  can be applied to perturb files  to ``trick'' a detector \cite{ling2021adversarial}, although the focus is to develop the AML techniques rather than evaluate commercial detectors. 
Notably, Fleshman et al. \cite{fleshman2018static} test four commercial antivirus (AV) technologies and self-made ML classifiers on perturbations of malware. 
Similar to this study, time constraints limit Fleshmen et al. to a corpus of 1,000 malware files, and further limitations are noted: ``all the malware ... has been known for some time and likely been used by the AV companies in their product updates.''
Overall, the results exhibit that the two (not commercial) ML-based classifiers are more robust to adversarial perturbations than the four commercial detectors.


VirusTotal\footnote{\url{www.virustotal.com}} (VT) is a leading threat intelligence source that tracks malware and provides determinations of 65+ commercial detection engines  for any submitted file.  
Previous work has involved VT data on files to study commercial malware detection engines. 
Zhu et al. \cite{zhu2020measuring} track labels (benign/malicious) through VT of these 65+ vendors for more than 14K files over time and focus on the label dynamics. 
% according to VT, and how accurate using the a threshold on statistics (e.g., if greater than 50 of 65 engines vote malicious, label malicious) is.
A primary finding is that commercial detection engines represented on VT are finicky, changing detection results often; nevertheless,  categorizing files based on a threshold voting schemes can be reliable for many thresholds that are intermediate in magnitudes. 
A portion of the paper uses files for which Zhu et al. know ground truth (benign/malicious) and is most related to our study. 
Specifically,  Zhu et al. create 120 zero-day ransomware samples (60 obfuscations of two known ransomware) and 236 benignware samples to test the commercial engines through VT. 
Observations include that detection rates are better over time, but for these samples, true positive \textit{and false positive} rates vary from approximately 25--100\%--which indicates wide variation in the commercial tools but also much worse precision than found in our study. 
Finally, Zhu et al. compare desktop version of 36 AV technologies against their VT counterparts, finding VT versions have on average higher recall but more false positives. 

Prior works have evaluated the efficacy of open-source network-based intrusion detection systems (IDSs), specifically Snort, Suricata, and Zeek~\cite{shah2018performance,murphy2019comparing,thongkanchorn2013evaluation}. Although these are commonly used in SOCs, they are not malware detectors. 


\subsubsection{Market Reports by Companies} 
\label{sec:market-reports}
\hl{Market reports are used by security operations to learn about products in the cyber technology marketplace; although these are not peer-reviewed academic research, we include information on relevant market reporting companies to provide context.
%% Nixing Gartner b/c irrelvant -- no evaluations!
Gartner (\hbox{\url{gartner.com/en/information-technology}}), a popular provider of market reports for the cyber technology space, curates market summaries composed of company profiles of the vendors, ratings and comments from end users of the products, information from the vendors' white papers, and often scores on a ``magic quadrant,'' proving quantification of the technologies' ``ability to execute'' and ``completeness of vision'' {\cite{gartner-mq}}. 
% While some information if free\footnote{For example, see \url{https://www.gartner.com/reviews/market/endpoint-detection-and-response-solutions} a Gartner page on endpoint detection and response (EDR) technologies.}  paid subscriptions are required to access the full reports. 
% Overall, Gartner provides valuable feedback in terms of satisfaction from end users, 
Gartner does not provide any scientific testing of the efficacy of detection tools. 
}

\hl{
Evaluations of IDSs are provided by commercial companies {\cite{fleshman2018static}}. 
MITRE ATT\&CK provides an evaluation online {\cite{mitre}} in which they examined 21 IDS products against the APT3 and APT29 threat groups. 
This evaluation includes custom malware and alternate execution methods. 
However, both the APT29 and APT3 include only two scenarios, for a total of four attack scenarios, so very little malware is actually executed. 
These evaluations do not specifically focus on the capability of the tools under test to detect malware but rather on their capability to detect realistic attack campaigns at any stage of execution. 
AV-TEST (\hbox{\url{av-test.org}}) and SE Labs (\hbox{{\url{selabs.uk}}}) both provide ratings based on evaluations of the malware detectors.
Although AV-TEST and SE-Labs' endpoint test results provide a rich source of statistics, they have two  main drawbacks. 
First, evaluations are seemingly too easy, diminishing trust in the tests and inhibiting the tests' capabilities to differentiate the technologies. 
As an example, in the evaluation of April 2022 {\cite{av-test}}, of the 20 detectors evaluated, 17 receive a 6/6 protection rating, with the remaining three obtaining a 5.5/6. Digging deeper, we find that the reviewers claim the industry average for detecting zero-day files is 99.8\%. 
Similarly, the quarter 1 endpoint detector test from SE Labs {\cite{selabs-test}} finds the top (approximately ten) detectors achieve near perfect (above 99\% accuracy) in most tests. 
Comparing these results with our findings---where recall of any single detector is under ~60\% across all tested malware---we are skeptical of the differentiation power of the tests provided. 
The second drawback is inherent to statistical results; making sense and reasoning logically about  many diverse measurements for each tool is difficult and has been a problem for evaluation of cyber technologies more generally {\cite{iannacone2020quantifiable}}. 
Our work seeks similar tests for these tools but provides an approach that addresses these drawbacks by providing a variety of files to (hopefully) be sufficiently difficult and to use a cost-benefit framework to reason about many diverse measurements produced by experiments.  
}

\hl{
Notably, VT does not provide comparative analytics of detection engines {\cite{virustotal}}.
}
%, and the Anti-Malware Testing and Standards Organization (AMTSO)\footnote{\url{https://www.amtso.org}} provides standards for tests. 



% Multiple studies found that Suricata is more accurate than Snort for detecting malicious traffic, but that it also consumed more network resources~\cite{shah2018performance, murphy2019comparing}. 
% Shah and Isaac~\cite{shah2018performance} clarify this finding, noting that Snort detects a higher percentage of malicious traffic, but that it has a high FP rate. 
% Common metrics for comparison include accuracy (number of FPs), efficiency (processor and memory usage), and resiliency (number of lost or dropped packets). 
% While these works do not relate to malware detectors, we include them because they are evaluations of COTS IDS tools. 



\subsubsection{Malware Detection Method Surveys}
Myriad papers examine existing or proposed novel malware detection methods.
Because our work focuses on evaluating the efficacy of commercially available tools, we do not discuss these works in detail.
However, in this section, we provide references to several surveys that provide thorough overviews of this literature.
A number of well-cited surveys discuss malware detection methods generally~\cite{aslan2020comprehensive,idika2007survey, ye2017survey}, and others focus more narrowly on areas such as dynamic~\cite{or2019dynamic}, static~\cite{shalaginov2018machine, souri2018state}, and mobile~\cite{qamar2019mobile} malware detection.
In their recent survey of malware detection approaches, Aslan and Samet~\cite{aslan2020comprehensive} highlight several research challenges that remain open issues in the malware detection space, including the following that are particularly applicable to our work:  no detection method can detect all unknown malware, obfuscation might prevent malware from being examined by existing tools, and false positives (FPs) and false negatives (FNs) are a problem with existing approaches. 
In our research, we quantify these issues in existing tools and suggest ways they can be alleviated, such as by using multiple approaches in tandem. 

\subsubsection{Methods of Evaluation of Detectors}
We refer the reader to Iannacone \& Bridges \cite{iannacone2020quantifiable}, which provide a survey of evaluation methods for cyber defenses, in particular intrusion detectors. 
Trends other than the usual statistical metrics (e.g., recall, precision) include incorporating time of detection into IDS metrics \cite{garcia2014empirical} and cyber competition scoring frameworks \cite{red-team-article, doupe2011hit, patriciu2009guide, reed2013instrumenting, werther2011experiences, mullins2007cyber}.  
Several significant works on security cost modeling, such as the Security Attribute Evaluation Method \cite{butler2002security}, the Return on Security Investment model \cite{sonnenreich2006return, davis2005return}, and the Information Security Risk Analysis Method \cite{karabacak2005isram}, led to the general cost-benefit framework of Iannacone \& Bridges that we build upon in Section \ref{sec:cost-model}. 
\hl{ Kondakci {\cite{Kondakci_2009}}  provides a costs analysis for the spread of malware through a network using epidemic-inspired models, which is an interesting and worthwhile work but not appropriate for our setting.} 

\subsubsection{Polyglot Files}\label{rel:poly}
Polyglot files are valid as multiple file types.
For example, a file could be a valid joint photographic group (JPG) and a valid Java archive (JAR) file, or it could be a valid portable document format (PDF) and a valid hypertext preprocessor (PHP) file.
Malware detection methods often require the file type to be known, so a polyglot file is used to prevent the correct file type association to bypass the detection mechanism.
A large body of research exists related to exploiting systems using polyglot files~\cite{bratus2016fillory, bratus2017exploitation,albertini2015abusing,magazinius2013polyglots,wolf2010omg}, as well as online tutorials on creating polyglot files\footnote{\url{https://medium.com/swlh/polyglot-files-a-hackers-best-friend-850bf812dd8a}}. 
However, there is little research focused specifically on helping IDS systems handle polyglot files.
The majority of existing research is focused on the challenges of identifying malicious PDF files~\cite{nissim2015detection, carmony2016extract}.
Although solutions such as binwalk\footnote{\url{https://github.com/ReFirmLabs/binwalk}} can be used to help identify polyglot files, it is unclear why they have not been integrated into commercial tools. 
One possible reason is that using a tool such as binwalk would have a negative impact on throughput. 





==> beyond-the-hype-3 (2)/20-experimental-design.tex <==
\section{Experimental Design}
\label{sec:experiment}
To execute the experiments, we leveraged the NCR, an air-gapped research test bed equipped with state-of-the-art network and user emulation capabilities to facilitate the experiment \cite{ferguson2014ncr}. 
A variety of services were emulated, including email, website servers, and domain controllers, and they were used by emulated users both internal to the network and in the emulated worldwide web (external).  
\hl{We provide a network diagram in the Appendix (Figure} \ref{fig:network-diagram}). 

\hl{Traffic generation was provided on all client endpoint virtual machines (VMs) by the NCR Mantra soft
ware, a proprietary emulator built on Lariat {\cite{lariat}}. 
All clients had broadly similar traffic generation profiles and were configured to automatically and randomly browse websites (both internal and external), send and reply to emails, generate Microsoft (MS) Office documents, transfer files to and from file shares and Sharepoint sites, and run a preset list of other benign executables. All clients were set to a fixed diurnal schedule of increased daytime activity between the hours of 0700 and 1700 local time; activity outside of these hours was decreased by a factor of 10 (i.e., average inter-arrival time of traffic generation events was set to be 10 times as high).}

\hl{System time was synchronized between all devices except the network static appliance via NTP to the central NCR testbed time source. Every node with an in-band connection synchronized to an NTP server in the simulated Internet environment, which in turn connected to the central time source via the testbed control network; everything with only an out-of-band connection connected directly via the
control network to the same source. The network static appliance was supplied as a vendor-loaned server without administrative (root) access, which is required to change time settings; the offset of this appliance’s time vs. actual time was noted for compensation in after-action data analysis.
}

This environment enabled delivery of malware over the network to endpoints running the two host-level tools, so the network-level tools could (attempt to) reconstruct files from the packet stream and provide detection.  
In particular,  emulated internal and external websites, mail servers, and hosts were used to deliver files (both benign and malicious) to  internal clients through web download, email attachments, and direct connections, respectively. 


% All technologies were required to operate on-premises, that is, without connections outside the internal portion of the emulated network. 
\hl{The authors met with vendors of the technologies and configured the tools in advance of the NCR to ensure proper configuration. 
Configuration guides were used to duplicate the process at NCR, and, as a quality assurance check, detection results on a set of test files were confirmed to be identical before the experiment (with tools configured by the vendors) to  after setup in the NCR.} 
% Configuration of the four detectors under test were done according to installation guide provided by the vendor. 
All technologies operated on-premises, without connections outside the internal portion of the emulated network. 
%(see Figure \ref{fig:network}). 
Although both host-level tools provide pre-execution conviction and quarantine, for the purpose of the experiment all tools were set to alert only (not block/prevent) to permit complementary (\texttt{OR}) % and confirmatory (AND) 
analysis of multiple tools. 
All machines were time synchronized. 
For the network-level tools, a secure sockets layer (SSL) %(secure sockets layer)
``break-and-inspect'' decryption technology was \textit{not} added to this network. Files were delivered on unencrypted protocols as the goal was to test the detectors' capabilities to detect malware without dependency on the capabilities of the decryption technology. 
(In practice, under this configuration malware sent encrypted would almost certainly be opaque to these detectors. How such a decryption technology affects the network-level detector is out of scope for this work.) 

% See Figure \ref{fig:network}, giving more details.
% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{fig/ncr-network-diagram-sanitized.png}
%     \caption{Experimental network architecture depicted. 
%     In bottom ``Internal Network'' portion, note the top left subnet are the hosts running the signature-based detector above the subnet of hosts running the ML-based detector. 
%     Management servers for the two host-based tools reside in the bottom left subnet. 
%     The dotted ``SPAN'' allows the network-level detection servers (one static, one dynamic) to access a mirrored copy of traffic for file reconstruction and alerting.
%     Opposing Force (OPFOR) Attacking machines denote ``malicious’' IPs}
%     \label{fig:network}
% \end{figure*}

For this experiment we evaluated the endpoint detection on both Windows 7 and 10 for an endpoint (nonserver) host, although Linux hosts and servers were present. 
Windows 7 and  10 VMs were given 4 GB of RAM and 1 CPU core, along with a large disk drive for the installed operating system. 
RHEL6 VMs were given 1 GB of RAM and 1 CPU core, also with a large disk drive for storing the operating system and associated files.
These values reflect the amount of minimum memory needed to create a VM for the specific operating system, with both the Windows VMs requiring at least 4 GB and RHEL requiring only 1 GB. 
The test bed was controlled via orchestration infrastructure leveraging virtualization software and custom wrapping software to coordinate with the VMs and manage the VM life cycle. 
% Finally, each ``golden image'' of the cybersecurity technologies was instrumented with custom code to collect computational performance metrics, specifically, usage of the CPU (percent), memory (bytes), hard drive  (bytes), 
% and network input/output bandwidth (bytes). 





==> beyond-the-hype-3 (2)/24-malware.tex <==
The detection technologies were each exposed to 3,536 total files (2,554/982 = 72/28\% malicious/benign) of varying categories, including 32- and 64-bit  portable executables (PE32, PE64), MS  Office, PDF, JAR, and three unusual categories: APT (described subsequently), zero-day PE (Windows PEs believed to not be available publicly), and polyglot  (files that are valid as multiple file types, e.g., ZIP and PDF). 
Most malicious files were obtained through VirusShare\footnote{\url{https://virusshare.com/}}. 
Our polyglot categories should also be never-before-seen files, and at least one of the valid file types has malicious functionality; 
\hl{specifically, we combined malicious Java JAR files with GIF and JPEG files. 
Notably, one can leverage open-source software for polyglot creation} (\url{https://github.com/corkami/mitra}). 
The zero-day files were manufactured samples that never touched infrastructure with access to the Internet. 

The goal of the APT class was to create artifacts that exemplified common APT evasion tactics. This included using signed vs. unsigned executables, cloning the PE headers of common benign executables, and advanced in-memory characteristics. 
Cobalt Strike\footnote{\url{www.cobaltstrike.com}} provided a convenient way to test these features. 
Because Cobalt Strike is a known tool, we needed to minimize the risk that our artifacts would be discovered by generic Cobalt Strike signatures. 
To this end, we built a custom obfuscator for the samples in the APT class using the Cobalt Strike artifact kit. 
The artifact kit is effectively an API that allows users to change the way Cobalt Strike generates binary artifacts, allowing advanced users to more successfully evade AV technologies. 
As a quality assurance step, we built a named pipe bypass using the artifact kit and ensured that default samples (i.e., samples without any of the APT-like evasions) generated with this obfuscation were not detected by a fifth, commonly used malware detector. 
% We chose evading defender as our sanity check simply because it was an AV product that wasn't directly under test). 
With this obfuscation in hand, the APT class was created by combining that obfuscation with the various APT-like evasions available in Cobalt Strike. 
% None of the generated samples were detected by our fifth quality assurance detection ability. 
% While we cannot be sure that any detected  APT samples in our experiment were not identified by known signatures, 
For those APT samples that were correctly detected in our experiment, we cannot know if the correct detection was from a generic signature (that our obfuscator failed to evade) or if indeed the APT-like evasion tactic was correctly identified behaviorally. 
% \begin{figure}
\begin{wrapfigure}[12]{r}{.5\textwidth}
% \vspace{-.82cm}
    \centering
    \includegraphics[width=.5\textwidth]{fig/filetype-barchart.eps}
    \caption{File category percentages}
    \label{fig:tc2-filetype-pie}
    % \vspace{-.45cm}
\end{wrapfigure}
% \end{figure}
\subsection{File Samples}


Our experiment used an imbalanced class, that is, a smaller number of benign files than malicious. 
As the experiment involved instantiating an entire analysis environment and waiting up to two minutes for a detection decision on each file, time limitations forced our decision to limit the benign files. 
We biased the benign set to include a set of ``tricky'' benign samples generated and donated by researchers who developed the Hyperion tool \cite{prowell2016automatic, linger2013computing}. 
These benign files are mostly C/C++ compiled utilities and were often (incorrectly)  classified as malicious in Hyperion research. 
The rest of the benign files are standard office type documents, JAR files, RPMs, DEBs, and EXEs/MSIs. 


Overall, inclusion of nonpublic malware and benignware allows testing of the ML generalizability hypothesis---that it can correctly identify never-before-seen files, while the variety of malware allows examination of recall across file types and categories. 

 
% \begin{table}[h]
%     \centering
%     \caption{File Types Used}
%     \begin{tabular}{|l|l|}
%       \hline
%       File Type & Description \\
%       \hline \hline
%       \textbf{PE} & An executable file\\ \hline
%       \textbf{Zero-day} & A malicious executable not available in-the-wild\\ \hline
%       \textbf{APT} & An advanced persistent threat (APT) malicious executable \\ \hline
%       \textbf{MS Office} & A MicroSoft Office file (docx, pptx, etc)  \\ \hline
%       \textbf{PDF} & A portable document format file (Adobe) \\ \hline
%       \textbf{JAR} & An executable java archive \\ \hline
%     \textbf{Polyglot} & A file with multiple valid file headers \\ \hline
%     \end{tabular}
%     \label{tab:tc2results-filetypes}
% \end{table}





==> beyond-the-hype-3 (2)/26-tools.tex <==

\subsection{Tested Technologies} 
\label{sec:tools}
All technologies tested are established malware detection products from well-known companies in the cyber tech market place. 
The three ML-based tools used in the test are of type  host ML, network static, and network dynamic detectors. 
\hl{All ML technologies came pretrained.} 
A popular endpoint signature-based detector was used as the baseline. 
The endpoint ML detector claims to use no signatures; therefore, it allow us to compare signature-only to ML-only detection at at the host level. 
Two network-level tools provide ML-guided detection, but one is static and the other is dynamic.
To test their technologies, we agreed to keep the  vendors and their intellectual property confidential.



%beca they both use the same (Zeek) file carving mechanism (i think that's true--can you check?),
%(static tool uses both ML and signatures in a suite)
\textbf{Host-Level, Signature-Based Detector:}
This proprietary detection tool uses static code analysis to compare hashes and portions of the file's binary with signatures, known malicious/benign hashes, and code snippets. 
This standard approach for an AV tool promises high precision and fast detection but an inability to identify novel, even slightly changed malicious files. 
In general, porting of signatures to each host requires relatively large host memory usage but facilitates fast and computationally inexpensive detection. 

\textbf{Host-Level, ML Detector:}
This host-based AV tool promises pre-execution file conviction for certain file types. % and can stop or prevent a malicious program from running, although only alerting capabilities are used/tested in our experiment. 
The binary classification uses supervised ML trained on large quantities of both malicious and benign files. 
According to vendor reports, the product requires 150 MB of memory on each host and claims that detection incurs computational expense similar to that incurred by taking a hash. 

\textbf{Network-Level, Static, ML Detector:} 
The network-level, static detection tool was designed to  passively detect (not block) both existing and new/polymorphic attacks before a breach, on the wire, in near real time, with an on-premises solution.  
This technology centers on a binary (i.e., benign/malicious) classification of files and code snippets extracted from network traffic. 
All features of the reconstructed files and code snippets result from static analysis. 
This product's sensors sit at a tap between the firewall and switch and between the router and hosts and rely on a variety of open-source tools for both feature extraction and classification; that is, in addition to their proprietary ML classifier, open-source file conviction technologies are used. 

\textbf{Network-Level, Dynamic, ML Detector:} 
The network-level dynamic detector reconstructs files from the network data stream and, 
%assesses them in a sandbox environment that is either an on-premises server or a cloud service for analysis.  
using a central analytics server that resides either on-premises or in the cloud, builds both static and dynamic features by running the file in sandboxes and emulation environments for analysis. 
The vendor claims the tool accommodates many file types including executable, DLL, Mach-o, Dmg, PDF, MS Office, Flash, ISO, ELF, RTF, APK, Silverlight, Archive, and JAR. 
Features are then fed to a binary supervised classifier. 
Presumably, network-level and behavioral features are included as well. 
Detection timing was quoted as up to 20 s to a few minutes, which, based on vendor reports, is much (i.e., orders of magnitude) slower  than competitors, although most competitors use static analysis only. 
This highlights the fact that, as with the network-level static detector tested, this product is primarily for detection, not  prevention.

==> beyond-the-hype-3 (2)/30-statistical-results.tex <==

\section{Statistical Results}
\label{sec:stats-results}

Here, we provide the usual accuracy  and conviction time statistics in aggregate, broken down by file type, and, for the network-level tools, by  delivery protocol. 
Furthermore, we present results for each detector side by side and in complementary combinations.  

\subsection{Individual Sensor Results} 
Table \ref{tab:tc2:comparative-analysis} itemizes the results of each malware analysis technology, with rows per file type except the bottom row, which gives overall detection statistics. 
Because a focus of this experiment is to identify the ways in which ML-based technologies add value, we consider the host signature-based sensor as a baseline.  
The host signature-based tool demonstrates perfect precision but poor recall, pulled down  by its inability to detect never-before-seen malware (0\% polyglots, 3.5\% zero-days detected). 
The tool performs relatively well with respect to MS Office files and APT files and fairly well with respect to executable and PDF files.  
Good performance on executable, MS Office, and PDF file types is not surprising because these are the most common packaging for malware and, therefore, have the broadest set of signatures.  
As expected, the host signature-based tool performed poorly on JAR files and zero-day samples, where there are fewer relevant signatures, or in the case of zero-day samples, no existing signatures. 


The good performance on the APT category was a surprise.  
It is likely that the Cobalt Strike %command and control 
framework used for packaging the APT malware samples just happens to be well known to the signature set used in this host signature-based sensor. 
The host signature-based tool's perfect precision simplifies this analysis, as recall becomes the primary metric of comparison.
Performing worse in overall recall, the host ML tool has 0\% detection for all non-PE files. 
The two network-level tools perform quite similarly, with good ($>$95\%) precision and both with better (but still alarmingly poor) recall of 55\%, giving F1 near 70\%. 

%%%%%%%%%%%%%%%%%%
The network static tool %uses a suite of ML- and signature-based subclassifiers to make determinations. 
% This approach allows it to 
achieves a recall of $\smalltilde$20\% greater than the host-based tools. 
As this tool uses a suite of ML- and signature-based subclassifiers, these results suggest that complementary signature and ML tools might work well.   
This increase in recall is shadowed by a higher quantity of FP alerts.   
Nearly identical overall statistics are achieved by the lone dynamic tool. 
\hl{Our results imply that network-level tools  do  increase recall substantially with comparable precision to the host ML tool and only slightly worse precision to the host static tool.}


Overall, regarding Table \ref{tab:tc2:comparative-analysis}, there is no clear ``winner.''
Precision values are high for all four tools, meaning all sensors performed with relatively few false alerts.  
Perhaps the biggest takeaway of these results is the utter failure of these tools to detect most malware. 
Recall of 33--55\% is both disappointing and alarming, with roughly 37\% of the malware used in the exercise undetected. Furthermore, recall varies wildly across file categories for each tool. 
Notably, most operations use a sole endpoint detector, and both of these state-of-the-art commercial detectors identified only a third of the malware used in this test. 
% A more comprehensive study of endpoint detectors is warranted to quantify, in a more statistically significant manner, the state of malware detection in practice. 
Polyglots are a glaring problem for these four tools, as no such file was detected. 
This suggests that the approach to detection is dependent on determination of file type. 

Considering the zero-day category, we see that all three ML-based tools (host ML and both network tools) increase recall by more than a factor of ten. 
This quantifies our first hypothesis, at least for these tools, that ML, as incorporated into modern detection products, can help generalize to never-before-seen files. 
Simply put, in our results, the detection rates increase by approximately ten times but at the cost of precision---specifically precision on PE32 files---which drops by approximately 10\%.  
% Any elation is prematurely dampened by the overall detection rates in the 33--55\% ranges.}
Considering only the zero-day PEs and the APT files, the network dynamic tool is (unsurprisingly) superior. 
% This is unsurprising as it is the only tool that sees the actions of the files. 
Comparing this result with the amount of time needed to detect will put these figures in context. 


%%%%%%%%%%%%%%%%%% Swarm of swarmplots!!!
\begin{figure}[t]
% \begin{wrapfigure}[45]{r}{.6\textwidth}
    % \vspace{-.2cm}
    \centering
    \includegraphics[width=.495\textwidth]{fig/host-signature-based-time-to-detect-with-alerts.eps}
    \includegraphics[width=.495\textwidth]{fig/host-ml-based-time-to-detect-with-alerts.eps}
    % \vspace{-.1cm}
    \includegraphics[width=.495\textwidth]{fig/network-static-time-to-detect-with-alerts.eps}
    \includegraphics[width=.495\textwidth]{fig/network-dynamic-time-to-detect-with-alerts.eps}
    \caption{Swarm plots show time to detection for each file type. Left plots show per-file-category results with blue/orange data for true/false alerts. Right plots show all file categories and depict the time-to-detection distribution.  
    \textbf{Top:} (Left) As the signature-based detector  has perfect precision, there are no FPs (no orange data points). (Right) Host ML detector does not detect many file categories and has many FPs in PE32 files. 
    \textbf{Bottom:} (Left) Network static detector has nearly identical time to detection for each file type except PE 32, the only type with false alerts, and all have relatively long analytic time. 
    (Right) The network dynamic detector has very few false alerts, but time to detect is one to two orders of magnitude longer. 
    }
    \label{fig:tc2:malware-analysis-times}
    % \vspace{-.7cm}
\end{figure}

\subsubsection{Detection Latency}
\label{sec:tc2:analysis-latency}
% \begin{figure}[ht]
%     \centering
%     % \includegraphics[width=\linewidth]{fig/tc2-did/MalwareAnalyzerTiming.png}
%     \includegraphics[width=\linewidth]{fig/cost-plots/time-to-detect-hist-bv.eps}
%     \includegraphics[width=\linewidth]{fig/cost-plots/time-to-detect-hist-juniper.eps}
%     \caption{ (Top) histogram of BluVector detection times, with average of 15.3s. (Bottom)  histogram of Juniper detection times, with average of 1039.0s.}
%     \label{fig:tc2:malware-analysis-times}
% \end{figure}

% An important element to the detection efficacy and in evaluating the cost of intrusions is the time to detect, or analysis latency, for a given technology.  
In addition to accuracy, timely detection is imperative to effective defense against malware.  
Figure \ref{fig:tc2:malware-analysis-times} shows each tool's time from file delivery until alert %(detection time in the case of a TP), 
both per file type with true and false positives (TPs/FPs) indicated by color and in aggregate across all files to visualize the overall alert time empirical distribution. \hl{Detection latency is calculated from the timestamp generated when the file transmission is completed until the timestamp of a given tool's alert on the respective file and encompasses all processing, including any file carving or decompression required.}
% gives histograms of conviction times for two of the malware analysis technologies, Network Static Tool (top) and Juniper (bottom). Conviction times for the tool range from approximately 11--19 s, whereas the conviction times for Juniper range from 1.5 minutes to over an hour. 
% It is important to note that because these are averages over all convicted files, outliers may skew the value.  Regardless, the average times give a good sense of relative latency associated with these tools.
Tools' average conviction times rank as expected, but the results hold some unexpected takeaways. 
The network static tool has the fastest average conviction time of 15.3s, perhaps due to the resources available for a network appliance (much more than an application on a host) and static technique (generally faster than dynamic detection). 
Interestingly, all its FPs occur in PE32 files that take maximum times to alert for this tool. (Without visibility into the detection mechanism of the tool, we cannot diagnose this phenomenon. We notified the vendors of this anomaly.)
% Extracting and transforming the file characteristics into a feature vector takes time, but the actual classification is typically quick. 
Both host-based tools take at most a couple minutes to alert, with the ML-based tool slower on average. 
Anomalously, the signature-based tool JAR files exhibit wide variance in time to alert. 
Recall that the host ML detector does not alert on many file categories and has many FPs on PE32 files, whereas the host signature-based tool has no FPs. 
The network dynamic tool has a \textit{much} greater average conviction time of 1,039 s. 
This is understandable given the process of creating a sandbox environment and then executing the file in that environment to make a conviction decision. 



We dug into the detection latency of these network-level tools in an additional experiment. 
Both vendors provided updated network appliances, and we tested their time-to-detect capabilities in a separate, more realistic experiment. 
Each tool received a mirrored feed of a real network's traffic blended with emulated network traffic, allowing more than 2,000 malware samples to be delivered safely to VMs but spread over a few hours. 
While seeing data rates of up to 7 GB/s, the tools achieved median detection times, 
\hl{ from file delivery until alert,} 
of under 1 s for the network static tool and 258 s = 4.3 m for the network dynamic tool. (Median is reported here because of outliers in the statistics that affected the mean.) 
The network-level tools had a significant bottleneck in the computational overhead of decompressing files. 
Introducing emulated network data had a positive effect on detection latency as it significantly decreased the rate at which compressed files were delivered to the tools despite dramatically increasing the amount of raw data to process---the tools received more network traffic but a decreased rate of compressed files to process.
These results show that, indeed, there is a latency cost for using at least this dynamic analysis tool and that both the network tools' latencies can increase by an order of magnitude if files cross the network too rapidly relative to the server's computational resources. 


\subsubsection{Network-Level Detectors Efficacy Across Protocols}
\label{sec:protocols}
\begin{wraptable}[]{r}{.33\textwidth}
% \vspace{-.3cm}
    \centering
    \caption{Detection counts for network-level detectors on 200 malware samples each sent on five protocols.}
    \label{tab:detection-across-protocols}
    \begin{tabular}{lcc}
        \toprule
          &  \textbf{Dynamic} &  \textbf{Static} \\
        \midrule
              FTP &      0/200 &        9/200 \\
             \rowcolor[HTML]{EFEFEF} HTTP &    145/200 &      156/200 \\
              SMB &      0/200 &       38/200 \\
             \rowcolor[HTML]{EFEFEF} SMTP &    180/200 &        N/A \\
              TCP &      0/200 &        0/200 \\
        \bottomrule
    \end{tabular}
\end{wraptable}
The two network-level tools rely on extracting files from traffic 
\hl{and claimed accommodation of multiple protocols. 
As such, we ran a small test using multiple protocols.} 
Our results revealed that visibility  into those network streams was not as reliable as expected. 
All of the 3,536 file samples used in the analysis were delivered over the HTTP protocol. 
To test the network tools' capabilities across protocols,  200 of the malware samples were also delivered over four additional protocols. \hl{To deliver files over multiple protocols, web downloads (HTTP), external file transfers (FTP), internal file transfer (SMB),  attachments to  emails (SMTP), and clear-text TCP via Netcat were used.  
Netcat was used to test a vendor's claim that it could detect files sent in this manner.} 
% This allows examination of the two network malware detectors across protocols. 
We present the counts of correctly detected samples for these 200 malware samples on the five total protocols in Table \ref{tab:detection-across-protocols}. 
The network static tool has an email client that was not used in this analysis, and so its performance on email was not determined. 
% To understand the technologies' performance at extracting files from network data streams, we conducted five tests for five different network protocols where 200 malware samples were transmitted through the network (visible to the network-based sensors) to an endpoint.  
All network transmissions were unencrypted. 
% The protocols evaluated included email, server message block (SMB), transmission control protocol (TCP), file transfer protocol (FTP), and HTTP. 
Both network IDS tools require de-/un-encrypted traffic. 
These results show that the tools' capabilities to detect varies greatly by protocol, and this does not include the complexity induced by the realistic assumption that  these tools would sit downstream of a companion decrypter.  


% Furthermore, recalling that network-level malware detectors generally do not prevent malware, as host-based tools do, the evidence suggests that network-level tools be considered only as complementary tools, enhancing host and other detectors, not lone malware defenses. 
% In short, despite the analytic value of network-based malware detectors, these technologies present a weakness in that any lack of visibility into network payloads will impair detection performance.












%%%%% old stuff
% In terms of F1 score comparison, the Network Dynamic tool, had the highest overall score with the Network Static tool  exhibiting a nearly identical score.
% Similarly, the results of Network Static Tool and Network Dynamic tool were both comparable in terms of recall. 
% the Host ML-Based Sensor had the worst performance in terms of F1, but overall results were skewed by the fact that the Host ML-Based Sensor only supports executable file types. 
% The Host Signature-Based Sensor  scored relatively low in terms of recall, but it had the distinction of perfect precision in this exercise, meaning that each alert produced by the Host Signature-Based Sensor was the result of an actual detected malicious file.
% Looking closer at Precision and \textit{Recall} values reveals some interesting characteristics. 
% the Host Signature-Based Sensor was perfect with respect to precision, which is not surprising given reliance on signatures. 



% provided better coverage in the PE32 PE64, JAR, and Zero-Day categories, and also provided good detection rates in Office files.  %This table provides no insight into whether the tools are all convicting the same files or whether the combined detection coverage is stronger than any one tool. This question will be addressed in the confirmatory and complementary analysis in Section \ref{sec:tc2:heterosensinganalysis}.  

% A glaring  hole in all tools' abilities was malware packaged in polyglot files, or files with multiple headers. 


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{fig/Filetype-f1-heatmap-anon.eps}
%     \caption{Malware Analyzer F1 Scores by File Type}
%     \label{fig:tc2:comparative-analysis-fscores}
% \end{figure}


% A summary statistic to gauge overall detection ability by category, the F1 score is computed for each tool. For ease of viewing, we visualize F1 results per filetype as a heatmap  in Figure \ref{fig:tc2:comparative-analysis-fscores}.
  
% Interestingly, while the Network Dynamic tool provides a much lower false positive rate, the F1 Score is overall not strikingly better than most of the others. 
%Interestingly, while the dynamic execution provides much lower false positive rate, the $F_1 Score$ does not vary much from the others. 
% Those technologies that do static classification are competitive with or outperform dynamic analysis in all categories.  
% Again, the F1 scores reported are comparative, and do not account for an complementary detection, and so there may be value in multiple detection approaches that is not immediately apparent in a side-by-side analysis.  
% The the Host ML-Based Sensor led the PE detection category, which included only already-in-the-wild malware. It also performed well on Zero-Day malware. 









% \begin{table}[ht]
%     \centering
%     \caption{Individual Sensor Results over all Malware Detection Tests}
% \begin{tabular}{lrrrrr}
% \toprule
%                   Tool &   TPs &  FPs &  Prec. &  Recall &    F1 \\
% \midrule
%  Host Signature-Based &   874 &    0 &      \textbf{1.0} &   0.342 &  0.51 \\
%  \rowcolor[HTML]{EFEFEF}        
%  Host ML-Based &   866 &   29 &  0.968 &   0.339 & 0.502 \\
%  Network Static &  1410 &   63 &  0.957 &   \textbf{0.552} &   0.7 \\
%  \rowcolor[HTML]{EFEFEF}      
%  Network Dynamic &  1386 &    7 &  0.995 &   0.543 & \textbf{0.702} \\
% \bottomrule
% \end{tabular}
% \label{tab:tc2:detector-summary}
% \end{table}

% \begin{table}[ht]
%     \centering
%     \caption{Individual Sensor Results over all Malware Detection Tests}
%     \begin{tabular}{lrrrrr}
%     \toprule
%           Tool &   TPs &  FPs &  Prec. &  Recall &   F1 \\
%     \midrule
%           HBSS &   874 &    0 &  \textbf{    1.0} &   0.342 &  0.51 \\
%         Cylance &   866 &   29 &  0.968 &   0.339 & 0.502 \\
%       BluVector &  1410 &   63 &  0.957 &   \textbf{0.552} &   0.7 \\
%         Juniper &  1386 &    7 &  0.995 &   0.543 & \textbf{0.702} \\
%     \bottomrule
%     \end{tabular}
% \label{tab:tc2:detector-summary}
% \end{table}

% \begin{table*}[ht]
% \centering
% \caption{Individual Sensor Results per Filetype}
% \label{tab:tc2:comparative-analysis}
% \begin{tabular}{lllllllllllll}
% \toprule
% \textbf{Filetype} & \multicolumn{3}{c}{\textbf{HBSS}} & \multicolumn{3}{c}{\textbf{Cylance}} & \multicolumn{3}{c}{\textbf{BluVector}} & \multicolumn{3}{c}{\textbf{Juniper}} \\
% (\#mal./\#ben.) & Prec. & Recall &    F1 &   Prec. & Recall &   F1 &     Prec. & Recall &   F1 &   Prec. & Recall &   F1 \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
% \textbf{APT} (27/0)       &    1.0&   0.67 &   0.8 &      1.0&   0.63 & 0.77 &        1.0&    0.3 & 0.46 &      1.0&   0.56 & 0.71 \\
% \textbf{JAR} (525/200)    &    1.0&  0.089 &  0.16 &       0 &      0 &    0 &        1.0&   0.25 &  0.4 &      1.0&   0.21 & 0.35 \\
% \textbf{Office }(600/200) &    1.0&   0.78 &  0.88 &       0 &      0 &    0 &        1.0&   0.87 & 0.93 &      1.0&   0.73 & 0.85 \\
% \textbf{PDF} (600/200)    &    1.0&   0.51 &  0.68 &       0 &      0 &    0 &        1.0&   0.51 & 0.68 &      1.0&   0.56 & 0.72 \\
% \textbf{PE32} (600/200)   &    1.0&   0.51 &  0.67 &    0.92 &   0.85 & 0.89 &      0.81 &   0.69 & 0.75 &    0.98 &   0.64 & 0.78 \\
% \textbf{PE64} (582/182)   &    1.0&   0.23 &  0.38 &      1.0&   0.78 & 0.87 &        1.0&   0.83 & 0.91 &      1.0&   0.76 & 0.86 \\
% \textbf{Polyglot} (199/0) &     0 &      0 &     0 &       0 &      0 &    0 &         0 &      0 &    0 &       0 &      0 &    0 \\
% \textbf{Zero-Day} (403/0) &    1.0&  0.035 & 0.067 &      1.0&   0.49 & 0.65 &        1.0&   0.39 & 0.57 &      1.0&   0.55 & 0.71 \\
% \bottomrule
% \end{tabular}
% \end{table*}


==> beyond-the-hype-3 (2)/31-table1.tex <==
%%% big table 1: 
\begin{table*}[ht]
\caption{Individual sensor results itemized. \hl{Categories are disjoint in this table: all 403 zero-day files are PE32 files but are \textit{not} counted in the \textbf{PE32} row; similarly, all polyglot files are malicious JARs but are \textit{not} counted in the \textbf{JAR} row. The \textbf{Total} row provides the statistics computed on all files. }}
\begin{adjustwidth}{-2in}{-2in}
\centering
\label{tab:tc2:comparative-analysis}
\begin{tabular}{lllllllllllll}
\toprule
\textbf{Category} & \multicolumn{3}{c}{\textbf{Host Signature}} & \multicolumn{3}{c}{\textbf{Host ML}} & \multicolumn{3}{c}{\textbf{Network Static}} & \multicolumn{3}{c}{\textbf{Network Dynam.}} \\
(\#mal./\#ben.) &                 Prec. & Recall &    F1 &          Prec. & Recall &   F1 &           Prec. & Recall &   F1 &            Prec. & Recall &   F1 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
\textbf{APT} (27/0)       &                     1 &  0.667 &    0.8 &              1 &   0.63 & 0.773 &               1 &  0.296 & 0.457 &                1 &  0.556 & 0.714 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (325/200)    &                     1 & 0.0892 &  0.164 &              0 &      0 &     0 &               1 &  0.249 & 0.399 &                1 &  0.209 & 0.346 \\
\textbf{Office} (400/200) &                     1 &  0.782 &  0.878 &              0 &      0 &     0 &               1 &  0.873 & 0.932 &                1 &  0.735 & 0.847 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF} (400/200)    &                     1 &  0.512 &  0.678 &              0 &      0 &     0 &               1 &   0.51 & 0.675 &            0.996 &  0.565 & 0.721 \\
\textbf{PE32} (400/200)   &                     1 &  0.505 &  0.671 &          0.922 &  0.855 & 0.887 &           0.814 &   0.69 & 0.747 &            0.977 &  0.642 & 0.775 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (400/182)   &                     1 &  0.233 &  0.377 &              1 &  0.777 & 0.875 &               1 &  0.833 & 0.909 &                1 &  0.757 & 0.862 \\
\textbf{Polyglot} (199/0) &                     0 &      0 &      0 &              0 &      0 &     0 &               0 &      0 &     0 &                0 &      0 &     0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &                     1 & 0.0347 & 0.0671 &              1 &  0.486 & 0.654 &               1 &  0.395 & 0.566 &                1 &  0.553 & 0.712 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
\textbf{Total} (2554/982) &                     \textbf{1} &  0.342 &   0.51 &          0.968 &  0.339 & 0.502 &           0.957 &  \textbf{0.552} &   0.7 &            0.995 &  0.543 & \textbf{0.702} \\
% \textbf{APT} (27/0)       &                    1.0&   0.67 &   0.8 &             1.0&   0.63 & 0.77 &              1.0&    0.3 & 0.46 &               1.0&   0.56 & 0.71 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{JAR} (525/200)    &                    1.0&  0.089 &  0.16 &              0 &      0 &    0 &              1.0&   0.25 &  0.4 &               1.0&   0.21 & 0.35 \\
% \textbf{Office} (600/200) &                    1.0&   0.78 &  0.88 &              0 &      0 &    0 &              1.0&   0.87 & 0.93 &               1.0&   0.73 & 0.85 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{PDF} (600/200)    &                    1.0&   0.51 &  0.68 &              0 &      0 &    0 &              1.0&   0.51 & 0.68 &               1.0&   0.56 & 0.72 \\
% \textbf{PE32} (600/200)   &                    1.0&   0.51 &  0.67 &           0.92 &   0.85 & 0.89 &            0.81 &   0.69 & 0.75 &             0.98 &   0.64 & 0.78 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{PE64} (582/182)   &                    1.0&   0.23 &  0.38 &             1.0&   0.78 & 0.87 &              1.0&   0.83 & 0.91 &               1.0&   0.76 & 0.86 \\
% \textbf{Zero-Day} (602/0) &                    1.0&  0.023 & 0.045 &             1.0&   0.33 & 0.49 &              1.0&   0.26 & 0.42 &               1.0&   0.37 & 0.54 \\
\bottomrule
\end{tabular}
\end{adjustwidth}
\end{table*}






==> beyond-the-hype-3 (2)/31-table2.tex <==
% \newgeometry{martin=1in} %can change margins for the landscaped page by putting, e.g,. margin=1cm, in the braces. 
% \begin{landscape}


%% big table 2
\begin{table*}[t]
% \vspace{-.2cm}
\caption{\hl{Top half of table: itemized complementary malware detection results }  ($result(A \texttt{ OR } B)$). \hl{Bottom half of table: Difference of the first (lone, base, host) detector's  results in Table {\ref{tab:tc2:comparative-analysis}} from the paired complementary detectors' results  in the top half of this table}  ($result(A \texttt{ OR }  B) - results(A)$).} 
\begin{adjustwidth}{-2in}{-2in}
\centering
\label{tab:tc2:compl-analysis}
\begin{tabular}{llllllllllllllll}
\toprule
\textbf{Category } & \multicolumn{3}{c}{\textbf{HostSig$\cup$HostML}} & \multicolumn{3}{c}{\textbf{HostSig$\cup$NetStat}} & \multicolumn{3}{c}{\textbf{HostSig$\cup$NetDyn}} & \multicolumn{3}{c}{\textbf{HostML$\cup$NetStat}} & \multicolumn{3}{c}{\textbf{HostML$\cup$NetDyn}} \\
(\#mal/\#benign)  &  Prec. & Recall &    F1 &   Prec. & Recall &    F1 &   Prec. & Recall &    F1 &   Prec. & Recall &    F1 &   Prec. & Recall &    F1 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{APT} (27/0)       &                        1 &   0.67 &  0.8 &                            1 &   0.67 &  0.8 &                            1 &   0.67 &  0.8 &                          1 &   0.63 & 0.77 &                          1 &   0.63 & 0.77 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (325/200)    &                        1 &  0.089 & 0.16 &                            1 &    0.3 & 0.46 &                            1 &   0.25 &  0.4 &                          1 &   0.25 &  0.4 &                          1 &   0.21 & 0.35 \\
\textbf{Office} (400/200) &                        1 &   0.78 & 0.88 &                            1 &   0.93 & 0.96 &                            1 &   0.91 & 0.95 &                          1 &   0.87 & 0.93 &                          1 &   0.73 & 0.85 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF} (400/200)    &                        1 &   0.51 & 0.68 &                            1 &   0.57 & 0.73 &                            1 &   0.58 & 0.73 &                          1 &   0.51 & 0.68 &                          1 &   0.56 & 0.72 \\
\textbf{PE32} (400/200)   &                     0.93 &   0.91 & 0.92 &                         0.85 &   0.86 & 0.86 &                         0.98 &   0.83 &  0.9 &                       0.85 &   0.93 & 0.89 &                       0.92 &    0.9 & 0.91 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (400/182)   &                        1 &   0.82 &  0.9 &                            1 &   0.86 & 0.92 &                            1 &    0.8 & 0.89 &                          1 &   0.86 & 0.93 &                          1 &   0.81 &  0.9 \\
\textbf{Polyglot} (199/0) &                        0 &      0 &    0 &                            0 &      0 &    0 &                            0 &      0 &    0 &                          0 &      0 &    0 &                          0 &      0 &    0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &                        1 &   0.49 & 0.65 &                            1 &    0.4 & 0.57 &                            1 &   0.56 & 0.72 &                          1 &    0.5 & 0.67 &                          1 &   0.62 & 0.77 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{Total} (2554/982) &                     0.98 &   0.57 & 0.72 &                         0.96 &   \textbf{0.61} & 0.75 &                            \textbf{.996} &   \textbf{0.61} &\textbf{ 0.76} &                       0.96 &   \textbf{0.61} & 0.75 &                       0.98 &    0.6 & 0.75 \\
% \bottomrule
% \end{tabular}

% \vspace{.3cm}

% \end{landscape}
%  \restoregeometry

% \begin{tabular}{llllllllllllllll}
% \toprule
% \multirow{2}{*}{\textbf{Category}} & \multicolumn{3}{c}{\multirow{2}{2.85cm}{\textbf{Host Sig$\cup$Host ML $\Delta$ Host Sig}}} & \multicolumn{3}{c}{\multirow{2}{2.85cm}{\textbf{Host Sig$\cup$Net Stat $\Delta$ Host Sig}}} & \multicolumn{3}{c}{\multirow{2}{2.85cm}{\textbf{Host Sig$\cup$Net Dyn $\Delta$ Host Sig}}} & \multicolumn{3}{c}{\multirow{2}{2.85cm}{\textbf{Host ML$\cup$Net Stat $\Delta$ Host ML}}} & \multicolumn{3}{c}{\multirow{2}{2.85cm}{\textbf{Host ML$\cup$Net. Dyn $\Delta$ Host ML}}} \\
\cmidrule(lr){2-16}
\cmidrule(lr){2-16}
& \multicolumn{3}{c}{\textbf{HostSig$\cup$HostML}} & \multicolumn{3}{c}{\textbf{HostSig$\cup$NetStat}} & \multicolumn{3}{c}{\textbf{HostSig$\cup$NetDyn}} & \multicolumn{3}{c}{\textbf{HostML$\cup$NetStat}} & \multicolumn{3}{c}{\textbf{HostML$\cup$NetDyn}} \\
 & \multicolumn{3}{c}{\textbf{ $\Delta$HostSig}} & \multicolumn{3}{c}{\textbf{ $\Delta$HostSig}} & \multicolumn{3}{c}{\textbf{ $\Delta$HostSig}} & \multicolumn{3}{c}{\textbf{ $\Delta$HostML}} & \multicolumn{3}{c}{\textbf{ $\Delta$HostML}} \\
(\#mal/\#benign) &                                    Prec. & Recall &   F1 &                                     Prec. & Recall &    F1 &                                    Prec. & Recall &    F1 &                                      Prec. & Recall &     F1 &                                   Prec. & Recall &    F1 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{APT} (27/0)       &                                        0 &      0 &    0 &                                         0 &      0 &     0 &                                        0 &      0 &     0 &                                          0 &      0 &      0 &                                       0 &      0 &     0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (325/200)    &                                        0 &      0 &    0 &                                         0 &   0.21 &  0.29 &                                        0 &   0.16 &  0.24 &                                          1 &   0.25 &    0.4 &                                       1 &   0.21 &  0.35 \\
\textbf{Office} (400/200) &                                        0 &      0 &    0 &                                         0 &   0.15 & 0.08 &                                        0 &   0.12 & 0.07 &                                          1 &   0.87 &   0.93 &                                       1 &   0.73 &  0.85 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF} (400/200)    &                                        0 &      0 &    0 &                                         0 &  0.06 & 0.05 &                                  0 &  0.07 & 0.06 &                                          1 &   0.51 &   0.68 &                                       1 &   0.56 &  0.72 \\
\textbf{PE32} (400/200)   &                                   -0.07 &    0.4 & 0.24 &                                     -0.15 &   0.36 &  0.18 &                                   -0.02 &   0.32 &  0.23 &                                     -0.07 &   0.07 & 0 &                                 0 &  0.05 & 0.02 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (400/182)   &                                        0 &   0.59 & 0.53 &                                         0 &   0.63 &  0.55 &                                        0 &   0.56 &  0.51 &                                          0 &  0.09 &  0.05 &                                       0 &  0.04 & 0.02 \\
\textbf{Polyglot} (199/0) &                                        0 &      0 &    0 &                                         0 &      0 &     0 &                                        0 &      0 &     0 &                                          0 &      0 &      0 &                                       0 &      0 &     0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &                                        0 &   0.45 & 0.59 &                                         0 &   0.36 &   0.5 &                                        0 &   0.52 &  0.65 &                                          0 &  0.02 &  0.01 &                                       0 &   0.14 &  0.11 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{Total} (2554/982) &                                    -0.02 &   0.23 & 0.21 &                                    -0.04 &   0.27 &  0.24 &                                  0 &   0.27 &  0.25 &                                     0 &   0.27 &   0.25 &                                   0.01 &   0.27 &  0.25 \\
\bottomrule
\end{tabular}
\end{adjustwidth}
\end{table*}










%%%%%%%%%%%%%%%%
%  \textbf{Filetype } &   \multicolumn{3}{c}{\textbf{Host Sig.}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Host ML}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Static}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Dyn.}} &   \multicolumn{3}{c}{\textbf{All Four Sensors}} \\
% (\#mal/\#benign) & Prec. & Recall &    F1 &                Prec. & Recall &   F1 &                Prec. & Recall &   F1 &              Prec. & Recall &   F1 &            Prec. & Recall &   F1 \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
% \textbf{APT }(27/0)       &    1.0&   0.67 &   0.8 &                   1.0&   0.67 &  0.8 &                     1.0&   0.67 &  0.8 &                   1.0&   0.67 &  0.8 &                 1.0&   0.67 &  0.8 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{JAR} (525/200)    &    1.0&  0.089 &  0.16 &                   1.0&  0.089 & 0.16 &                     1.0&    0.3 & 0.46 &                   1.0&   0.25 &  0.4 &                 1.0&    0.3 & 0.46 \\
% \textbf{Office} (600/200) &    1.0&   0.78 &  0.88 &                   1.0&   0.78 & 0.88 &                     1.0&   0.93 & 0.96 &                   1.0&   0.91 & 0.95 &                 1.0&   0.93 & 0.96 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{PDF} (600/200)    &    1.0&   0.51 &  0.68 &                   1.0&   0.51 & 0.68 &                     1.0&   0.57 & 0.73 &                   1.0&   0.58 & 0.73 &                 1.0&   0.58 & 0.73 \\
% \textbf{PE32} (600/200)   &    1.0&   0.51 &  0.67 &                 0.93 &   0.91 & 0.92 &                   0.85 &   0.86 & 0.86 &                 0.98 &   0.83 &  0.9 &               0.85 &   0.94 & 0.89 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{PE64} (582/182)   &    1.0&   0.23 &  0.38 &                   1.0&   0.82 &  0.9 &                     1.0&   0.86 & 0.92 &                   1.0&    0.8 & 0.89 &                 1.0&   0.89 & 0.94 \\
% \textbf{Polyglot} (199/0) &     0 &      0 &     0 &                    0 &      0 &    0 &                      0 &      0 &    0 &                    0 &      0 &    0 &                  0 &      0 &    0 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{Zero-Day} (403/0) &    1.0&  0.035 & 0.067 &                   1.0&   0.49 & 0.65 &                     1.0&    0.4 & 0.57 &                   1.0&   0.56 & 0.72 &                 1.0&   0.63 & 0.77 \\
% \bottomrule

==> beyond-the-hype-3 (2)/32-complementary-results.tex <==
\input{31-table2}
\subsection{Complementary Detection}
\label{sec:tc2:heterosensinganalysis}

% While the comparative analysis helps us to better understand how tools performed independently, it does not provide insight into their ability to work together  coverage of the malicious/benign data sets. 
In light of the surprisingly low detection rates (33--55\%, see Table \ref{tab:tc2:comparative-analysis}), we consider simulated results of using pairs of tools together by taking the logical \texttt{OR} of binary classifiers. 
Tool pairs will score well if they alert on different malware---thereby increasing recall---but overlap on false alerts. 
Specifically, we consider pairing the two host-based detectors together to see if host signature and ML techniques are a good combination. 
Then, we consider combining each host tool paired independently with each network-level tool. See Table \ref{tab:tc2:compl-analysis}. 
% of the two host-based tools  host-based and ML-based malware detectors. % in order to understand the additive value of heterogeneous sensing combinations.  
% As these network-level tools provide malware detection but not prevention we do not recommen

% Most network-level malware detectors do not prevent (e.g. quarantine) detected files from executing on the host without communicating with a host agent. Secondly, the lack of robustness in extracting files correctly from a wide variety of network protocols (Section \ref{sec:protocols} is the limiting factor to adopting a network-centric endpoint malware analysis architecture.


% A subset of possible combinations for complementary ensembles are presented in this table including the Host Signature-Based sensor in combination with each of the ML-based tools, only network-based ML malware detectors, and then the use case of combining all sensor combinations.

% An examination of the improved recall scores is found in Table \ref{tab:tc2:compl-analysis}. 

Complementing the host signature-based tool with other technologies increases recall dramatically for PE32, PE64, and zero-days files. 
Precision of the host signature tool is minimally sacrificed only for PE32 files in these pairings. 
Similarly, as the host-ML tool does not alert on many file categories,  substantial gains in detection capabilities are possible by adding any other tool.
% Both host tools together or either host tool with one of the network tools.  
As a final baseline, we considered the union of all four tools (Table \ref{tab:all-four-unioned}), which only slightly increases recall with little change to precision over these pairs. 
In short, combinations of either the host-level tool with one other malware detector yields much better recall with little impact to precision, and only pairs of tools are needed---unioning three or more detectors provides little gain.
\begin{wraptable}[15]{r}{.4\textwidth}
\caption{\hl{
Results of complementary detection (logical union) of all four detectors.
}}
\centering
\label{tab:all-four-unioned}
\begin{tabular}{llll}
\toprule
\textbf{Category} & \multicolumn{3}{c}{\textbf{All Four Detectors}} \\
(\#mal/\#benign)  &          Prec. & Recall &   F1 \\
\cmidrule(lr){2-4}
\textbf{APT} (27/0)       &              1 &   0.67 &  0.8 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (325/200)    &              1 &    0.3 & 0.46 \\
\textbf{Office} (400/200) &              1 &   0.93 & 0.96 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF} (400/200)    &              1 &   0.58 & 0.73 \\
\textbf{PE32} (400/200)   &           0.85 &   0.94 & 0.89 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (400/182)   &              1 &   0.89 & 0.94 \\
\textbf{Polyglot} (199/0) &              0 &      0 &    0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &              1 &   0.63 & 0.77 \\
\cmidrule(lr){2-4}
\textbf{Total} (2554/982) &           0.96 &   0.67 & 0.79 \\
\bottomrule
\end{tabular}
\end{wraptable} 


% reveals that the ML-based sensors add significant value when combined with a signature-based sensor.  All three ML-based technologies significantly improve recall scores for executable categories (PE32, PE64 and Zero-Day PEs), and the network based ML technologies (Network Static Tool and Network Dynamic tool), boost the recall values across all file types except the APT and Polyglot categories.  

% The motivation behind including the combined complementary results of the network-based malware detection technologies, both static (Network Static Tool) and dynamic (Network Dynamic tool), was to postulate the efficacy of a cybersecurity architecture where malware analysis is performed exclusively at the network level.  
% In other words, we seek to quantify whether replacing endpoint malware analysis with both static and dynamic analysis at the network level improves malware detection.  
% As compared to the Host Signature-Based Sensor alone, it is a dramatic improvement.  
% However, our analysis revealed that malware sensors that carved files out of network data streams only performed well on two protocols: SMTP and HTTP.  


% In terms of recall, the Network Static Tool Cortex $\cup$ Juniper combination outperforms HBSS alone on every filetype category except for APT and Polyglots. It exhibits competitive Precision that is, on some filetypes, slightly below the perfect Precision exhibited by HBSS. 
% However, the efficacy of these network-based technologies requires visibility into the network payload to reconstruct network streams and their file contents.  
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.1\linewidth]{fig/complementary-filetype-f1-heatmap.eps}
%     \vspace{-.85cm}
%     \caption{Complementary F1 Scores by File Type}
%     \label{fig:tc2:complementary-analysis-fscores}
% \end{figure}




% Figure \ref{fig:tc2:comparative-analysis-fscores} provides a heatmap of the F1 scores for a quick visual analysis of the overall gain of adding each ML tool to the Host Signature-Based Sensor, and for considering all tools used together. 
%In order to see best detection performance for complementary heterogeneous sensing combinations, considering both Recall and Precision, Figure \ref{fig:tc2:complementary-analysis-fscores} shows and compares F1 Scores for each file type and for each sensing combination.  

% As with Table \ref{tab:tc2:compl-analysis}, the Host Signature-Based Sensor is included as the lower bar for each file type as a basis of comparison. This graphic conveys the improvement of combining analytic modes of sensing, with the addition of ML-bases sensors to the signature-based sensor providing a substantial improvement in most categories. The combination of all sensors provides the highest F1 score across all categories, but combining the analytics of the the Host Signature-Based Sensor with either the static or dynamic network-based malware classifiers appears to give the strongest dual-sensor performance. The host-based malware classifier (the Host ML-Based Sensor) has the highest performance on in-the-wild PE files, but is limited with respect to file types covered and so adds less complementary value as a general malware detection capability.
% By definition, adding a complementary sensor can only increase recall. Since All Four Sensors has maximal or near maximal F1, we see that precision is not decreased much by complementary unions. 
% Network Dynamic tool shows overall the strongest single tool addition to the Host Signature-Based Sensor. 
% Compare these results with the estimate in Section \ref{sec:savings-addition} of savings from adding a network-level detector. 



==> beyond-the-hype-3 (2)/34-confirmatory-results.tex <==

\begin{table*}[t]
    \centering
    \caption{Confirmatory malware detection results by file category}
\begin{tabular}{llllllllllllllll}
\toprule
 \textbf{Category } &   \multicolumn{3}{c}{\textbf{Host Sig.}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Host ML}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Static}} &   \multicolumn{3}{c}{\textbf{Host Sig.} $\cup$ \textbf{Net. Dyn.}} &   \multicolumn{3}{c}{\textbf{All Four Sensors}} \\
(\#mal/\#benign) & Prec. & Recall &    F1 &                Prec. & Recall &   F1 &                Prec. & Recall &   F1 &              Prec. & Recall &   F1 &            Prec. & Recall &   F1 \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
\textbf{APT} (27/0)       &    1.0&  0.667 &    0.8 &                   1.0&   0.63 &  0.773 &                     1.0&  0.296 &  0.457 &                   1.0&  0.556 &  0.714 &                 1.0&  0.296 &  0.457 \\
\rowcolor[HTML]{EFEFEF}
\textbf{JAR} (525/200)    &    1.0& 0.0892 &  0.164 &                    0 &      0 &      0 &                     1.0& 0.0431 & 0.0826 &                   1.0& 0.0462 & 0.0882 &                  0 &      0 &      0 \\
\textbf{Office} (600/200) &    1.0&  0.782 &  0.878 &                    0 &      0 &      0 &                     1.0&  0.728 &  0.842 &                   1.0&  0.613 &   0.76 &                  0 &      0 &      0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PDF }(600/200)    &    1.0&  0.512 &  0.678 &                    0 &      0 &      0 &                     1.0&  0.448 &  0.618 &                   1.0&  0.497 &  0.664 &                  0 &      0 &      0 \\
\textbf{PE32} (600/200)   &    1.0&  0.505 &  0.671 &                   1.0&  0.455 &  0.625 &                     1.0&   0.33 &  0.496 &                   1.0&  0.318 &  0.482 &                 1.0&  0.273 &  0.428 \\
\rowcolor[HTML]{EFEFEF}
\textbf{PE64} (582/182)   &    1.0&  0.233 &  0.377 &                   1.0&  0.188 &  0.316 &                     1.0&  0.205 &   0.34 &                   1.0&  0.193 &  0.323 &                 1.0&  0.168 &  0.287 \\
\textbf{Polyglot} (199/0) &     0 &      0 &      0 &                    0 &      0 &      0 &                      0 &      0 &      0 &                    0 &      0 &      0 &                  0 &      0 &      0 \\
\rowcolor[HTML]{EFEFEF}
\textbf{Zero-Day} (403/0) &    1.0& 0.0347 & 0.0671 &                   1.0& 0.0347 & 0.0671 &                     1.0& 0.0298 & 0.0578 &                   1.0& 0.0298 & 0.0578 &                 1.0& 0.0273 & 0.0531 \\
\bottomrule
\end{tabular}
    \label{tab:tc2:conf-analysis}
\end{table*}



\subsection{Confirmatory/Corroborating Sensors}
\label{sec:confirmatory}
In addition to understanding how different sensing tools are complementary, it is useful to understand the extent to which they corroborate each other. 
Note that we use the term ``corroborate" and ``confirm" interchangeably. 
In a diverse sensing environment, confirmatory sensors may provide context as to the severity of an event or reliability of a malware detection.  
In terms of cybersecurity architecture, it can also reveal those sensors that duplicate detection capability.  
Table \ref{tab:tc2:conf-analysis} is a confirmatory analysis of various sensing combinations.  
Similar to complementary analysis, confirmatory analysis considers sensor combinations, but it differs in that it evaluates \textit{intersection} rather than the union of their individual detection results. In analyzing the confirmatory results of sensing combinations, it is interesting to note that the Host Signature-Based Sensor combined with any of the ML-based technologies results in poorer detection performance overall.  
This indicates a low degree of intersection between detection using the signature-based methods vs. the ML-based methods. 
In some cases, such as with MS Office and PDF files, for the Host Signature-Based Sensor $\cap$ Network Static Tool  and PDF files for the Host Signature-Based Sensor $\cap$ Network Dynamic tool, the recall value remains close to their comparative values, indicating that these combinations of tools are assessing malware files consistently for those file categories. 
Given the high precision of the evaluated malware detection technologies, it does not add value to consider them in a confirmatory way, given that their detections are complementary. 

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/confirmatory-filetype-f1-heatmap}
    \caption{Confirmatory $F_{1} Scores$ by File Category}
    \label{fig:tc2:confirmatory-analysis-fscores}
\end{figure}

An interesting result is the consistency between the union and intersection of the network-based malware analyzers; for most categories, drop-off is minimal regardless of whether these tools are considered in a complementary or confirmatory way. Thus, despite the different modes of sensing (static and dynamic malware analysis), these technologies are assessing malware very consistently and are largely a duplication of capability.
Considering precision and recall together, Figure \ref{fig:tc2:confirmatory-analysis-fscores} shows the F1 scores for all pair-wise combinations of sensors and all file categories, when looking at their corroborating detections.  
% As with previous heatmaps and tables, the Host Signature-Based Sensor  is included alone  as a baseline.  
%As noted in the discussion of Table \ref{tab:tc2:conf-analysis}, the combination of Network Static Tool Cortex $\cap$ Juniper JATP had the overall highest F1 Scores, indicating that these two tools have highly similar analytic value. That is, they are assessing files very similarly.




==> beyond-the-hype-3 (2)/40-cost-model.tex <==
\section{Cost Model Evaluation}
\label{sec:cost-model}
Although the aforementioned metrics provide a valuable statistical summary of these sensors' performance, recent work by Iannacone \& Bridges \cite{iannacone2020quantifiable} provides a cost--benefit framework that models the real-world implications of using a particular tool, yielding a single, comparable cost metric to more easily reason out the tradeoffs implied in Section \ref{sec:stats-results}.
% Our goal in this section is to provide a cost--benefit analysis of the two network-based malware detectors. 
% Explicitly, it is evident from the basic statistics of the detection experiment that the 
For example, the network dynamic tool has an average detection time of 1,039.0 s, an FP rate of 0.71\%, and a TP rate of 54.3\%, whereas the network static tool detects on average in 15.3 s (faster) with an FP rate of 6.42\% (worse) and TP rate of 55.21\% (about the same). 
It is difficult to know which tool is best for a given SOC to adopt based on these basic statistics. 
It is even more difficult to choose the best pair of tools. 


To assist with these determinations, we configured the cost 
model to evaluate these tools as standalone detectors (Section \ref{sec:result-one-tool}). This follows the original cost-model work \cite{iannacone2020quantifiable} but makes one novel contribution to the basic model. Since the cost model as originally proposed depends on the accuracy statistics of the tool, we test with a relatively large number of both malicious and benign files to accurately estimate these inputs.
Our change to the model is to compute average costs per benign-/malware, then scale the costs to respect two new model inputs, namely the expected number of files per year times the ratio of benign-/malware expected in the wild. 
This allows us to gain accuracy in both the detection  statistics and the cost model. 
In Section \ref{sec:savings-addition} we  create a new version of the model to compute savings of adding a network-based malware detector, assuming a host-based detector is in place. 
This new estimate is created to answer (Q2). 
\begin{wraptable}[12]{r}{.33\textwidth}
    % \vspace{-.3cm}
    \centering
   \centering
   \caption{Initial (one-time) server or appliance and ongoing (annual) subscription costs.}
    \begin{threeparttable}
    \begin{tabular}{lcc}
    \toprule
    & \textbf{Initial} & \textbf{Ongoing}\\
    \midrule
     Host Sig.  & \$2K  & \$8K/y \\ 
    \rowcolor[HTML]{EFEFEF}  Host ML  & \$6.5K & \$35K/y\\
     Net. Static & \$15K & \$20K/y\\
    \rowcolor[HTML]{EFEFEF}  Net. Dynam.  & \$23K & \$16K/y\\
    \bottomrule
    \end{tabular}
    \end{threeparttable} 
    \label{tab:cost-estimates}
\end{wraptable} 





% \begin{wraptable}[12]{r}{.35\textwidth}
%     \vspace{-.3cm}
%     \centering
%   \centering
%   \caption{Initial (one-time) \& ongoing (annual) resource costs.}
%     \begin{threeparttable}
%     \begin{tabular}{c lr}
%     \toprule
%      {}  & \multicolumn{2}{c}{\textbf{Resource}}\\
%       \cmidrule{2-3}
%      \multirow{4}{*}{\rotatebox{90}{\textbf{Initial}}}
%      {} & Host Sig. Server & \$2K  \\
%      {} & Host ML  Server & \$6.5K\\
%      {} & Net. Static Server & \$15K\\
%      {} & Net. Dynam. Appliance & \$23K\\
%      \cmidrule{2-3}
%      \multirow{4}{*}{\rotatebox{90}{\textbf{Ongoing}}} 
%      {} & Host Sig.  Subscription  & \$8K/y \\ 
%      {} & Host ML Subscription & \$35K/y\\
%      {} & Net. Static Subscription & \$20K/y\\
%      {} & Net. Dynam. Subscription & \$16K/y\\
%     \bottomrule
%     \end{tabular}
%     \end{threeparttable} 
%     \label{tab:cost-estimates}
% \end{wraptable} 
% as well as adding a network-based to a host-based tool (Section \ref{sec:savings-addition}), predicting absolute costs and savings, respectively. 
%To assist with this question, we configured the cost model to evaluate both network-level tools as stand-alone detectors under a variety of attack cost scenarios, and consider them in conjunction with each host-based detector, to determine the costs or savings predicted by the model. 

% As most samples tested were malware, we researched the malware-to-benignware distribution observed in real world data and in the cost model scaled the results to to satisfy a realistic malware-to-benignware distribution.  
% % Subsection \ref{sec:malware-distribution} discusses our implementation of the cost model, designed to use all test samples while scaling estimates to satisfy a realistic malware-to-benignware distribution. 
% Recalling that 200 samples were sent multiple times on different protocols, we used only the HTTP-delivery of each sample in this section.

% This model estimates the incurred costs for using the tool, including (a)  initial resource and labor cost for deploying and then maintaining the technology and (b) labor and resource cost for alert triage, incident response (IR), and attack damages.
% %Note that these triage and incident response costs depend on the detection accuracy metrics discussed previously.
% % This model also includes the estimated costs of attack damages, which depend on the time needed to detect them.  
% To estimate the costs, we (a) use the costs of needed software and hardware and consult SOC operators for resource estimation and (b) leverage the statistical detection results (i.e., precision, recall, time to detect) and the inputs of domain experts (SOC operators), as well as existing literature to map these experimental results to a real-world SOC setting. 
% Fig. \ref{fig:attack-cost} displays attack costs over time used for our model, while Table \ref{tab:cost-estimates} itemizes resource costs. 
% Labor costs were estimated identically per tool at 8hrs initially, and for ongoing tuning monthly. 
% Triage of incurred a \$.05 resource cost for SIEM indexing plus a 1 labor hour per alert. 
% Finally, IR cost incurred 4hr labor per true alert. 
% We used a fully-burdened per labor estimate of \$70/hr for all labor costs.  

% %% This paragraph drops a bunch of names instead of doing an actual lit review
% %% possibly revisit?
% %%% Excluded GL model b/c it's really an upper bound estimate on how much you should spend. 
% %, and the Gordon-Loeb (GL) Model\cite{gordon2002economics,gordon2015externalities}, as well as the Mean Time to Compromise estimate researched by Leversage and Byres\cite{leversage2008estimating}.
% %Discussion of drawbacks and their mitigation
% % While this is an improvement on these earlier methods, this cost metric does share one common limitation---

% While this cost metric offers an objective way to weigh these trade-offs, the main limitation is 
% a dependence on inputs that are difficult to estimate and can be highly subjective. 
% % The attack damage costs are potentially the most difficult to estimate, 
% % but there are also several network- and organization-specific costs which must be estimated,
% % such as the incident response time, the quantity of files scanned, traffic volumes, etc. This metric provides a total cost in dollars, but if these inputs are incorrect, the resulting cost estimate may not accurately reflect the real-world cost of each tool's use. 
% However, there are two main mitigations that can restore confidence in using these estimates in this evaluation setting. 
% %comparative evaluation. 
% First, the parameters that are the most difficult to estimate are revealed in analysis to be the ones that have the least impact on cost results. 
% The initial work of Iannacone \& Bridges \cite{iannacone2020quantifiable} provides a sensitivity analysis of this method, which identifies the inputs that are most critical and indicates that the triage, incident response, and attack costs are the most important; 
% hence, we pay more attention to accurately modeling these costs (see Section \ref{sec:labor-rec-param})
% % To estimate these, we interviewed a SOC lead and cybersecurity expert who verified and provided input for our estimates of these costs. %, shown in Table \ref{tab:cost-estimates}.  
% % We note there are several important latent variables that effect the costs from triage, IR, and attack costs\textemdash namely, the true and false positive rates and the time to detection for each tool. 
% % These latent variables are not estimated, but obtained directly from the NCR experimental data. 
% % Next, we compute results as we vary those impactful parameters over a range of realistic values to obtain more robust comparison. 
% Furthermore, we compare overall costs from the model with the analogous figures from recent reports that estimate actual, real-world, recent costs of malware \cite{accenture-cost} to make sure overall outputs are of the right scale.
% % We also note that to have reasonable estimates, the ratio of benignware to malware must be close to real-world values. 
% % Our implementation seeks to match the real-world malware distribution described in recent research by Li et al. \cite{li2017large}, which examines this ratio. 
% Second, while absolute costs output by the model may not reflect real-world costs, we are most interested in a comparative evaluation---that is, the relative costs and rankings of the tools. Conducting a sensitivity analysis in Section \ref{sec:result-vary-params} illustrates that for overly large ranges of values, the least well-motivated parameter estimates ($N$, $M$, $\alpha$) do not effect tool rankings. 
% To verify that the relative costs given by the model are realistic, we implement and compare the full model outputs on simple baselines (i.e., no detection, always alert, perfect and immediate detection), demonstrating that the order and scale of the results are reasonable. 



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% % \begin{table*}[t]
% %   \centering
% %   \caption{Resource and labor cost estimates (cost model inputs)}
% %     \begin{threeparttable}
% %     \begin{tabular}{l lr c lr c c}
% %     \toprule
% %     %  \multirow{1}{*}{\rotatebox{90}{\textbf{IR}}} 
% %      {}  & \multicolumn{2}{c}{\textbf{Resource}} && \multicolumn{2}{c}{\textbf{Labor}} && \textbf{Frequency} \\
% %       \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-8}
% %      \multirow{4}{*}{\textbf{Initial}}
% %      {} & Host Sig. - Management Server & \$2K    && \multirow{4}{*}{Initial Configuration} & \multirow{4}{*}{8hrs $\times$ \$70/hr} && \multirow{4}{*}{once} \\
% %      {} & Host ML - Management Server & \$6.5K\\
% %      {} & Network Static - Server & \$15K\\
% %      {} & Network Dynamic - Appliance & \$23K\\
% %      \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-8}
% %      \multirow{4}{*}{{\textbf{Ongoing}}} 
% %      {} & Host Sig.  - Subscription  & \$8K/y && \multirow{4}{*}{Tuning} & \multirow{4}{*}{8hrs/mo $\times$ 12mo $\times$ \$70/hr} &&  \multirow{4}{*}{annually} \\ 
% %      {} & Host ML - Subscription & \$35K/y\\
% %      {} & Network Static - Subscription & \$20K/y\\
% %      {} & Network Dynamic - Subscription & \$16K/y\\
% %      \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-8}
% %      \multirow{1}{*}{{\textbf{Triage}}} 
% %      {} & SIEM Indexing & \$0.05 && Analyst time (ave.) & 1hr $\times$ \$70/hr && per alert \\
% %      \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-8}
% %      \multirow{1}{*}{{\textbf{IR}}} 
% %      {} & N/A &\$0 && Analyst time (ave.) & 4hr $\times$ \$70/hr && per true positive \\ 
% %     \bottomrule
% %     \end{tabular}
% %     \end{threeparttable} 
% %     \label{tab:cost-estimates}
% % \end{table*} 

==> beyond-the-hype-3 (2)/42-cost-model-overview.tex <==
\subsection{Cost Model Overview}
\label{sec:cost-model-description}
\label{sec:malware-costs}
This model estimates and sums labor and resource costs incurred for buying, configuring, and using the tool in  
addition to attack damage cost estimates. These costs are itemized by the following components. Refer to Table \ref{tab:cost-estimates}.

\textbf{$C_I$, the one-time initial costs of purchases, setup, and installation.} 
The initial configuration costs are based on our team’s experience with installing and configuring these devices at the NCR. All costs are slightly obfuscated to preserve anonymity of the tool vendors. 
This minimally impacts results but does not impact the rankings of the tools. All license, hardware, and labor costs assume a relatively small network ($\smalltilde$1K IPs), comparable in size and complexity to the NCR test network described previously. Note that we ignore several smaller costs, such  as power and cooling, because they are negligible. 




\textbf{$C_B$, the ongoing (per month, year, etc.) costs of normal operation,} including subscription-based licenses and labor needed for periodic updates, reconfiguration, and maintenance. Since we did not use the tools in a real setting for a long period of time, we simply cannot give per-tool estimates. We assumed 8 h/tool/month for all tools. This does not affect our comparison  and was included for completeness. 


\textbf{$C_{IR}$, the incident response (IR) cost (per true positive alert),} representing labor costs for investigation and remediation of detected attacks. 
We estimate this at \$280 = \$70/h (fully burdened cost of SOC operator) $\times$ 4 h.

\textbf{$C_T$, the alert triage costs (per alert),} representing labor costs and storage costs for the alert’s data. We
\begin{wraptable}[]{r}{.33\textwidth}
% \vspace{-.3cm}
    \centering
    \caption{Cost model parameters}
    \label{tab:cost-model-params}
    \begin{threeparttable}
    \begin{tabular}{ll}
        \toprule
          \textbf{Param. Value} & \textbf{Description} \\
        \midrule
             $M$ =    \$2,000  &        Max. Attack Cost \\
             \rowcolor[HTML]{EFEFEF} 
             $\alpha$ =  15m = 900s & Half-Cost Time \\
              $N$ = 125K& \# of Files\\
             \rowcolor[HTML]{EFEFEF} 
             $r$ = 1.16\%& Malware Ratio\\
        \bottomrule
    \end{tabular}
    \end{threeparttable}
\end{wraptable} 
estimate this at \$70/h $\times$ 1 h. 
A SOC lead verified that these estimates of labor time for triage and (above for) IR were verified as reasonable. 
The triage resource cost of \$0.05 was obtained by finding the lowest volume Splunk license based on the rate of raw data being processed (\$1,800 for 1 GB/month, or 34 MB/day) and estimating what fraction of that volume would  be consumed by each alert. 
For both detectors, we observed a peak of 1,000 alerts per day during our testing, and the average alert size was under 1 KB per alert, for a maximum of 1 MB/day. Because each detector is using less than 1/34th of the licensed volume for its 1,000 alerts per day, each alert represents a cost of (at most) \$1,800/34/1,000 or about \$0.05. 




$C_A$: While the above four costs are ``defense costs,'' $C_A$ \textbf{estimates the losses due to attack damages.} Attack cost is a function  of time modeling the average cost incurred from the moment of infection. 
\hl{We follow formulation of attack cost from the initial work {\cite{iannacone2020quantifiable}} and  use an ``S'' curve to model average attack cost over time. The intuition is that costs will begin at \$0 and after some time (e.g., the malware unpacking itself) begin to grow quickly, then level out approaching a maximum cost. 
In reality, this might happen in a sequence of discrete jumps, but as discussed in the previous work, an ``S'' curve provides a reasonable model of the average cost for an attack.}
Specifically, the attack damage cost $f(t)$ is defined as:
% \begin{equation}
% \label{eq:attack-cost}
$f(t) = M \exp(-  (\alpha/t)^2 \ln{2}) = M  2^{-1/(t/\alpha)^2}$
% \end{equation} ,
where parameter $M$ is the maximum cost (and horizontal asymptote), and parameter $\alpha$ is the time when half the maximum cost is attained ($f(\alpha) = M/2)$). 
See depiction of $f(t)$ in Figure \ref{fig:attack-cost} and input parameter choices 
in Table \ref{tab:cost-model-params}. 
The shape of the attack cost function, the parameters in Table \ref{tab:cost-model-params}, and the cost of labor hours used in this model were informed by discussions with a SOC lead who verified they are reasonable. 

% \begin{figure}[!b]
\begin{wrapfigure}[]{r}{.5\textwidth}
    \centering    
    % \vspace{-.3cm}
    \includegraphics[width=.5\textwidth]{fig/attack-cost.eps}
    \centering
    \caption{Attack cost model, \small{$f(t) = M  2^{-1/(t/\alpha)^2}$}}
    \label{fig:attack-cost}
    % \vspace{-.2cm}
\end{wrapfigure} 


% We discussed the attack damage cost with a SOC team lead 
% from a large government organization who agreed the ``S'' curve defined was an appropriate model. 
% To estimate $M$,  he noted that potential damage costs vary widely; %, spanning many orders of magnitude.
% many samples simply do not execute properly or may only perform menial actions (e.g., changing the default homepage) giving $M \approx 0$; 
% some samples can cost a medium amount in damages (e.g., traditional ransomware)  on the order of \smalltilde\$1K, including work hours lost, time to restore data, and related costs; finally, malware leading to a large data breach may result in in multi-million dollar losses, although such a campaign requires is generally not attributable to a single malware. 
% %used as ingress for an advanced persistent threat (APT), malware can cost millions, by exfiltrating sensitive data and placing footholds throughout the network, resulting in extreme incident response cost time. 

% To estimate the half-cost time $\alpha$, we note that nearly all malware begins by executing a series of necessary preliminary steps (e.g., unpacking itself, attempting to escalate privileges, enumerating host resources, performing reconnaissance, attempting to download auxiliary malware, and/or contacting a command and control server)  before it can work towards its goal. 
% If malware is detected and stopped before this point, it will have caused little to no monetary damage. 
% After this initialization period, however, the malware would begin to make costly maneuvers,  including potentially ex-filtrating data, corrupting data, spreading laterally (which increases remediation costs), and causing a denial of service. 
% Our SOC liaison guessed that an average of 10 min is a reasonable estimate for the time it takes most malware to complete the preliminary steps (and thus to begin incurring monetary damages), but he cautioned that some exploits may wait for 2--3 days to begin spreading, not incurring any damage for a few days, but an attack would likely incur penalties of much greater magnitude thereafter. 
% In light of this discussion, we use $M =$\$2K and $\alpha = 15$ m = 900 s in our analysis and results in Sections \ref{sec:result-one-tool} (see Table \ref{tab:cost-results}) and \ref{sec:savings-addition} (see Table \ref{tab:cost-add-to-host}), while in Section \ref{sec:result-vary-params}, we vary $M$ and $\alpha$ (see Figure \ref{fig:vary-params}) to investigate the impact of the choice of the $M, \alpha$ parameters on results. 



==> beyond-the-hype-3 (2)/46-implementation.tex <==
% \subsection{ Cost Model Implementation}
% \label{cost-model-implementation}
% Our goal was to test the cost-benefit evaluation method above on all of the test samples. 

To apply the model we first computed initial and ongoing costs, as explained previously, then compute each tool's cost per sample as follows:%, which are independent of detection performance. 
\begin{description}
\item[False Negative Costs: ] If the tool does not alert on a malicious sample, maximum attack cost is incurred ($M = \lim_{t\to\infty} f(t)$).
%($M = \lim_{t\to\infty} f(t) = \lim_{t\to\infty} M  2^{-1/(t/\alpha)^2}$) is incurred. 
\item[True Positive Costs:] If the tool correctly detects malware in $t$ seconds, the incurred cost is the sum of costs from triage resource and labor ($\$0.05 + \$70$), IR labor ($\$280$), and attack damages $f(t)$. 
Very late detection of malware can cost more than no detection because, for large $t$, the attack cost is near maximal, and alert triage and remediation still occurs.  
\item[False Positive Costs:] If the tool incorrectly alerts on a benign sample, triage costs are incurred ($\$0.05 + \$70$).
\item[True Negative Costs: ] If the tool (correctly) does not alert on benignware, no extra costs are incurred. 
\end{description}
%%%%%%%%%%%
% \begin{table}[ht]
% \centering
% \caption{Results of Static vs. Dynamic NIDS \& three baselines on two attack scenarios}
% \label{tab:cost-results}
% \begin{threeparttable}
% \begin{tabular}{lcrccrcc}
% \toprule
%   &&& \multicolumn{2}{c}{$M = \$5$K, $\alpha = 15$m} & & \multicolumn{2}{c}{$M = \$500$K, $\alpha = 2.5$days}\\
%   \cmidrule{4-5} \cmidrule{7-8}
%   &  Ave. Benign. Cost &&  Ave. Malware Cost &  1 Year Cost &&   Ave. Malware Cost &   1 Year Cost \\
%   \cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8}
% \textbf{Network Dynamic}                &                   \$0.50 &&            \$3,464.87 &  \$5,132,029.99 &&          \$228,638.39 & \$331,633,637.60 \\
% \rowcolor[HTML]{EFEFEF}
% \textbf{Network Static}              &                   \$4.49 &&            \$2,430.87 &  \textbf{\$4,122,274.95} &&                             \$223,939.49 & \textbf{\$325,309,774.95 }\\
% Never Alert              &                   \$0.00 &&            \$5,000.00 &  \$7,292,280.00 &&                            \$500,000.00 & \$725,042,280.00 \\
% \rowcolor[HTML]{EFEFEF}
% Always Alert &                  \$70.05 &&              \$350.05 &  \$9,204,530.00 &&                               \$350.05 &   \$9,204,530.00 \\
% Perfect Detector          &                   \$0.00 &&              \$350.05 &    \$549,852.50 &&                                 \$350.05 &     \$549,852.50 \\
% \bottomrule
% \end{tabular}
% \end{threeparttable}
% \end{table*} 
%%%%%%%%%%%


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{fig/vary-total-files-anon.eps}
%     \caption{Cost model results when varying the total number of files. This verifies that the total number of files simply linearly scales each detector's cost results, and demonstrates that the ordering of tools in terms of costs does not differ based on the total number of files per year.}
%     \label{fig:vary-total-viles}
% \end{figure}
Note that FN and TP costs are costs from malicious samples, whereas FP and TN costs are from benign samples. 


\hl{We break up the sum of $C_{IR} + C_T + C_A$ (incident response, triage, and attack costs) into two quantities---costs from false alerts plus from attacks (true alerts or no alert). 
To do so, we compute each tool's average benignware cost $a_b$  (from the remaining 992 benign samples) and average malware cost $a_m$ (from the 2,554 malware samples). 
% Finally, from talking to a SOC operator, we estimated the number of unique files crossing the network detector (border traffic + internal-to-internal) for a 1,000 IP network at about %on the order of 1 file per person per work day or 
% 125K files per year. 
Finally, we set $N$, the number of unique files crossing the network detector (border traffic + internal-to-internal) for a 1,000 IP network, to be 125K files (125 per host).
We also need an estimate of the ratio of malware to benignware in the wild. For this we leverage Li et al. {\cite{li2017large}}, who upon investigating files on 10K IPs find 1.16\% malware and 98.84\% benignware.
} 
Thus, we can scale the average cost per benign 
or malicious file to 125K files per year, respecting the 98.84/1.16\% benign-/malware ratio. 

\hl{Putting it all together, the \textit{estimated cost for the first $y$ years is:} }
\begin{align} 
\label{eqn:cost}
    C   &= C_I      &&\text{initial resource and labor costs plus} \nonumber \\
        &+ y[  &&\text{years ($\times$ quantity)} \nonumber  \\
        &  \phantom{+ y[ + } C_B && \text{yearly ongoing costs, e.g., subscriptions and tweaking, plus} \\
        &   \phantom{+ y[ } + N \times 98.84\% \times a_b && \text{annual costs from false alerts, plus} \nonumber \\
        &  \phantom{+ y[ } + N \times 1.16\% \times a_m] && \text{annual costs from attacks (end quantity)} \nonumber 
        % & \phantom{+ y[ }] \nonumber
\end{align}

            
                    % n_hard * ave_hard_malware_cost +  ## yearly cost of hard attacks
                    % n_easy * ave_easy_malware_cost + ## yearly cost of easy attacks
                    % n_benign * ave_benign_cost  ## yearly cost of false positives



Importantly, $N$ linearly scales all costs except the initial and ongoing costs (see in Figure \ref{fig:vary-params} (Left)), so unless the initial and ongoing costs for a tool are exorbitant, inaccuracies in this file number estimate will not affect any comparison of the tools.
For the latter two, we assumed detection was ``immediate'' using a detection time of $t = 1\mathrm{E}{-10}$~s. 

%See Figure \ref{fig:vary-total-viles}.  



%This was already explained above:
%The true positive rate and the time to detection are the influence of the tool on its incurred cost from malware, and each false positive rate is the tools' influence on its incorrect cost from benignware. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> beyond-the-hype-3 (2)/48-results.tex <==
% \begin{table}[t]

\subsection{Single-Tool Cost Model Results}
\label{sec:cost-model-results}\label{sec:result-one-tool}
For comparison in the subsequent results, we include three simulated  detector devices: ``Never Alert,'' which simulates no detector; ``Always Alert,'' which alerts on every file; and a ``Perfect Detector,'' which correctly alerts on only malware.
\begin{wraptable}{r}{.5\textwidth}
% \vspace{-.33cm}
    \centering    
\caption{Cost model results---mean cost per benign-/malware ($a_b$ , $a_m$) and 1st year cost---with three simulated baselines using parameters as in Table \ref{tab:cost-model-params}. Cost increases linearly in per-file costs. Mean benignware cost is a multiple of the false alert rate, while resp. mean malware cost is monotonically related to the recall and time to detect via attack cost function.}
\label{tab:cost-results}
\begin{threeparttable}
\begin{tabular}{lccc}
\toprule
{} &  Benign & Malware & first  1st Year\\
\cmidrule{2-4}
Host Sig.       &            \$0.00 &          \$1,435.47 & \$2,098,712\\%.95 \\
\rowcolor[HTML]{EFEFEF}
Host ML               &             \$2.07 &          \$1,440.54 & \$2,393,151\\%.55 \\
Network Dyn.      &            \$0.50 &          \$1,500.41 & \$2,283,562\\%.28\\
\rowcolor[HTML]{EFEFEF}
Network Static   &               \$4.49 &          \$1,089.10 & \$2,176,719\\%.15 \\
\midrule
Never Alert             &             \$0.00 &          \$2,000.00 & \$2,942,280 \\
\rowcolor[HTML]{EFEFEF}
Always Alert &            \$70.05 &            \$350.05 & \$9,204,530 \\
Perfect Detector              &             \$0.00 &            \$350.05 &   \$549,852 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{wraptable}
% \end{table}

% \subsubsection{Single Tool Cost Results}
Table \ref{tab:cost-results} displays the average benign-/malware costs and the estimated cost of using each tool alongside the simulated baseline under parameters as shown in Table \ref{tab:cost-model-params}. 
First and foremost, the simulations provide validation of the model, as all tools perform much better than the always alert simulation (accruing enormous false positive cost but minimal true positive cost) and much worse than the perfect detector device.
Because malware is relatively rare (ratio of 1.16\%), the cost of never alerting, though still more than all actual detectors, is closer than the other two simulated baselines. 
The tool rankings show that the host signature tool is superior because it has no FPs and competitive time to detect. 
As we only consider the host tools for realistic standalone defenses, we note that even with identical initial and ongoing costs, the host \hl{signature-based} tool is superior.
Interestingly, the network static detector places second because it is by far the fastest detector and has high recall, both outweighing its higher FP rate (high Ave \$/Benign). 
The network dynamic tool is hindered by its slow detection time (Figure \ref{fig:tc2:malware-analysis-times}) but benefits from accuracy. 

% \begin{wrapfigure}[35]{r}{.6\linewidth}
\begin{figure*} 
% \vspace{-.1cm}
\centering    
    % \includegraphics[width=\linewidth]{fig/vary-M-all-models.eps}
    \includegraphics[width=.48\linewidth]{fig/vary-M-zoom-intersections.eps}
    \includegraphics[width=.48\linewidth]{fig/vary-alpha-M2000.eps}
    % \includegraphics[width=1.05\linewidth]{fig/vary-params-subplots}
    \caption{Cost model results for varying $M = $ maximum attack cost with half-cost time $\alpha = 15$m (left); varying $\alpha$ with $M =\$2000$  (right).  Regarding the \hl{left} plot,  for $M$ near 0, it is cheaper to never detect (never alert baseline is cheapest). For $M \in [\smalltilde\$300, \smalltilde\$2300]$ the host signature detector is best and is second to the network static tool for $M>\smalltilde\$2300$.  Regarding the \hl{right} plot, for small (large) $\alpha$, attack cost accrues quickly (slowly), with the effect that slow  detection will be very (not very) penalized. The lone dynamic tool is very slow to detect but very accurate; hence, with large $\alpha$ it dominates. Of the two host-based tools, the signature-based method wins for nearly all parameters.}
    \label{fig:vary-params}
    % \vspace{-.5cm}
\end{figure*}
\subsubsection{Insights from Varying Cost Model Parameters}
\label{sec:result-vary-params}
% This model allows us to combine the many statistical results discussed in Section \ref{sec:stats-results} into a concise ranking of the tools based on simulated usability costs. 
The skeptic might object to  cost-benefit analyses, citing that, especially for cybersecurity applications, such methods suffer from required inputs that are fundamentally difficult to ascertain \cite{iannacone2020quantifiable, butler2002security};  and, indeed, our model is no different. 
% e.g., parameters $M$ and $\alpha$ give attack cost over time which is difficult to estimate. 
To account for these unknowns, this section investigates parameter sensitivity.% to test robustness of the results above.  


% While this cost metric offers an objective way to weigh these trade-offs, the main limitation is a dependence on inputs that are difficult to estimate and can be highly subjective. However, there are two main mitigations that can restore confidence in using these estimates in this evaluation setting. First, the parameters that are the most difficult to estimate are revealed in analysis to be the ones that have the least impact on cost results. The initial work provides a sensitivity analysis of this method, which identifies the inputs that are most critical and indicates that the triage, incident response, and attack costs are the most important \cite{iannacone2020quantifiable}; hence, we pay more attention to accurately modeling these costs. 
% Furthermore, we compare overall costs from the model with the analogous figures from recent reports that estimate actual, real-world, recent costs of malware \cite{accenture-cost} to make sure overall outputs are of the right scale. 
% Second, while absolute costs output by the model may not reflect real-world costs, we are most interested in a comparative evaluation—--that is, the relative costs and rankings of the tools. 
% Conducting a sensitivity analysis in Sec. \ref{sec:result-vary-params} illustrates that for a large ranges of values, the least well-motivated parameter estimates $(N, M, \alpha)$ do not effect tool rankings. 

Costs for all tools scale linearly in $N$, the number of files, so this will not change rankings. 
Cost increases linearly with mean \$/benignware with weight $N\times (1-r)$ and mean \$/malware with weight $r$, where $r$ is the malware ratio. 
Ave\$/benign is a multiple of the false alert rate,  while Ave\$/malware is monotonically related to the tool's recall and time to detect via attack cost. 
Thus, increasing/decreasing $r$ decreases/increases impact of the false alert rate but increases/decreases the impact of recall and time to detect. 
Precision directly affects results, but recall's effect depends indirectly on $M$ and $\alpha$. 
To investigate, we present costs while varying $M$ and $\alpha$ in Figure \ref{fig:vary-params}. 
The main takeaway is that the host signature tool is the best standalone choice based on these results and cost model. 
It offers the lowest cost for nearly all values of $M$ and $\alpha$, and otherwise (Figure \ref{fig:vary-params}) is second to network tools. 
% Given network tools are not stand-alone tools, our results suggest signature-based malware detection is best.


\begin{figure*} 
% \vspace{-.1cm}
\centering    
    % \includegraphics[width=\linewidth]{fig/vary-M-all-models.eps}
    \includegraphics[width=.48\linewidth]{fig/vary-hfc.eps}
    \includegraphics[width=.48\linewidth]{fig/vary-hfr.eps}
    % \includegraphics[width=1.05\linewidth]{fig/vary-params-subplots}
    \caption{\hl{Cost model results for varying $M_{hard} = $ maximum attack cost for hard files (namely polyglot, zero-days, and APT-style files) with percent of hard malware $p=0.05$ (left) and varying $p$ the percent of malware that is hard with $M_{hard} = \$20,000$ (right). 
    In both, the same half-cost time $\alpha = 15$ m is used for all malware, and for easy malware, $M =\$2,000$. 
    First notice that both plots are similar in structure because of the linear nature of these variables---both increases in $M_{hard}$ and $p$ convert savings from those with low recall  to those with better recall on hard files. 
    Hence, in both plots, we see that for small values of $M_{hard}$ and $p$ the signature-based detector wins; for intermediate values, the network static (relatively faster detection, competitive recall) wins; yet for larger values, the host ML and network dynamic (best recall on hard files) win. These results are intuitive, which is reassuring, but force a difficult reality; that is, deciding which tool is best depends on one's estimate of the hard'' malware expected. This suggests pairing signature- and ML-based tools. }}
    \label{fig:vary-params-hard}
    % \vspace{-.5cm}
\end{figure*}
\subsubsection{Insights from Increasing Cost of ``Hard'' Files---Zero-days, Polyglots, and APT-style Files} 
Another addition to the original cost model that is applicable to this study is increasing the cost of the ``hard'' malware: zero-days, polyglots, and APT style files, representing the assumption that such files, if undetected,  will result in more damage than $n-$day files, on average. 
To exhibit results under these conditions,  we compute  $a_{mh}$ the average hard file cost using the detection times on only the zero-days, polyglots, and APT-style functions and with augmented maximum attack cost $M_{hard}$ (still using the same equation with identical $\alpha$).
Similarly, we compute $a_{me}$, the average ``easy'' file cost identically on the remaining ($n-$day) malware detection results and using a maximum attack cost of $M = \$2K$.
Finally, we replace the final line of Equation \ref{eqn:cost} (namely, $N \times 1.16\% \times a_m$ ) with a convex sum of  the average cost from hard malware files and from easy malware files (namely, $N\times 1.16\% \times p  \times a_{mh} + N\times 1.16\% \times (1- p)\times a_{mh}$) using a parameter $p$, the percent of malware assumed to be hard. 
Results are depicted in Figure \ref{fig:vary-params-hard}. 
The main takeaway is that if one expects (1) more than a couple percent of malicious files to be a zero-day, polyglot, or APT-style file and (2)  the cost from an undetected hard file to be much greater than otherwise, ML-based detectors provide substantial savings. 



\subsection{Savings by Adding Network Detectors}
\label{sec:savings-addition}
Here we describe a new way to configure the cost model that is likely more useful for real-world use---estimating the cost/savings of adding each network malware detector to each host-based detector. 
% Assuming that an endpoint detector is in place, we only incur costs/savings from adding the network tool will be incurred. 
To do so, we add the initial and ongoing costs for the network tool then compute the difference in cost between using both the host-based and network-based tools and solely the host-based tool.  
As before, we (1) compute the additional cost/savings per file, (2) find the average cost/savings per malware file and per benignware file, and (3) linearly scale these costs/savings to 125K total files, respecting the 98.84/1.16\% benign-to-malicious file ratio. 
To estimate the change in cost on a given file, if the network   tool  does not alert on a given sample, 
there is no change in cost. 
%%%%%%%%%%%
\begin{wraptable}[10]{r}{.66\textwidth}
% \begin{table}[t]
% \vspace{-.75cm}
\centering
\caption{Cost on average per file and for first year of network detection tools  when added to each host-based detector individually. Negative costs indicate savings.}
\label{tab:cost-add-to-host}
\begin{threeparttable}
\begin{tabular}{lcrccrcc}
\toprule
&&& \multicolumn{2}{c}{\textbf{Host ML}} & & \multicolumn{2}{c}{\textbf{Host Signature}} \\
 \cmidrule{4-5} \cmidrule{7-8}
{} &  Benign &&  Malware &  1st Year  &&    Malware &  1st Year \\
\cmidrule{2-2} \cmidrule{4-5} \cmidrule{7-8}
\textbf{Dyn.}   &               \$0.50 && \$-145.26 &         \textbf{\$-102,651}%.40} 
&&                          \$-298.22 &               \textbf{ \$-324,443}%.61 }
\\
\rowcolor[HTML]{EFEFEF}
\textbf{Stat.} &               \$4.49 &&         \$-434.09 &          \$-31,913%.58 
&&                          \$-427.36 &                 \$-22,148\\%.51 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{wraptable} 
%%%%%%%%%%% 
If the network tool alerts on a sample (FP or TP), then triage resource and labor costs ($\$0.05 + \$70$) are incurred, accounting for an operator fielding the alert from the network tool (possibly in addition to alerts from the host-based detector). 
Moreover, if this network-based alert is a TP, and the host-based tool also correctly alerts on the sample, we make no other change to costs for this file; only triage cost is added for the network alert. 
This follows two assumptions: (1) IR actions will have taken place with or without the network-based alert since the host-based tool correctly alerted and (2) host-based detection is at least as fast as the network detector, resulting in no change in attack cost. 
These assumptions are based on the fact that most host-based tools offer \textit{pre-execution file conviction} and \textit{blocking}. %, resulting in alerts but no IR costs, these assumptions seem reasonable. 
As the final case, consider when the network tool's alert is a TP but the host-based tool failed to alert on the malware. 
In this scenario, without the network-based tool, the attack goes undetected, and the maximum attack cost is incurred. Yet with the network-based tool, there are now triage and IR costs, but the attack cost is reduced from maximal to $f(t)$, the attack cost at $t = $ the network-level detection time. 
In our model, this is the lone scenario in which savings from the network-level tool can occur---when the network tool identifies malware that is undetected by the host tool and the network tool identifies it fast enough that the change in attack cost is lower than the incurred triage and IR costs. 


Table \ref{tab:cost-add-to-host} reports the results of adding both  network-based tools to the two host-based detectors with parameters as in Table \ref{tab:cost-model-params}.  
% For this analysis we used the ``normal'' attack scenario described above with maximum attack cost $M = \$2,000$, and half-cost time $\alpha = 15$m. 
Reassuringly, both network-level detectors yield substantial (\$22K--\$325K) savings when added to the host tools. 
% Interestingly, the static network malware detector averages more cost savings per malware sample than the dynamic tool, and provides nearly double the savings when added to the host ML tool compared to when adding the dynamic network tool to the host ML tool.
% Yet, the high false positive rate of the static network-level tool renders it slightly less economical than the dynamic tool when added to the host signature-based detector.  
These results predict that, for SOCs using either host detector, dynamic detection is the best pairing, saving  3--15$\times $ more than the static detector. 









% is much cheaper than the dynamic detector. Due to the much lower time to detection for static vs. dynamic (see Fig. \ref{fig:tc2:malware-analysis-times}, bottom four subplots), the dynamic network tool incurs much lower lower average malware costs, which outweighs the fact that the static detector has more false alerts than the dynamic detector (evidenced in the higher Ave. Benign Cost for the static detector, and the results in Table \ref{tab:tc2:comparative-analysis}).  
% Using our worst-case, APT scenario for all malware (max. cost, $M = \$500,000$ and half-cost time, $\alpha = 2.5$days) the static detector still wins,  achieving now only slightly lower cost score; in this case  the longer half-cost time (large $\alpha$) in the malware cost model mitigates the dynamic tool's long average time to detection, making the overall costs relatively close.  

% (Top) we can make a few observations. 

% We note that the Never Alert baseline model performs best when the max cost $M$ is very low. 

% In those cases it's cheaper to simply let the malware incur the maximum cost instead of paying for triage and IR.  
% Similarly, for extremely high malware costs, the best strategy is always alerting immediately, paying triage costs for every benignware but eliminating the (extreme) expense of any malware. 
% Intuitively, the Never Detect baseline wins on the far left and Always Detect is second only to the Perfect Detection model on the far right.

% Fig. \ref{fig:vary-params} (Bottom) is simply a close-up on the intersection of the two network detectors and the Never Alert simulation.
% As mentioned above, if malware costs are very small, e.g., below about ~\$700, it is simply cheaper to never alert than to use either network detection tool. 
% Yet, there is an intermediate cost of malware, $M\in [\smalltilde\$700,  \smalltilde \$1,700]$ where the dynamic detector is better than the static detector and better than never alerting, caused by the fact that it is a more accurate detector (about 10\% of the false positives of the static detector). 
% For $M>\smalltilde\$1,700$, the long detection time of the dynamic tool renders the statit network malware detector the better option. 




% \begin{figure}[ht]
%     \centering
%     \vspace{-.5cm}
%     \includegraphics[width=\linewidth]{fig/vary-alpha-M2000.eps}
%     % \includegraphics[width=\linewidth]{fig/vary-alpha-M500000.eps}
%     \vspace{-.5cm}
%     \caption{
%     Cost model results for varying half-cost time, $\alpha $.
%     Top plot fixes maximum attack cost, at  $M = \$5,000$ and considers $\alpha $ from 0 to 80m (normal attack scenario), while the bottom plot fixes $M = \$500,000$ and varies $\alpha$ on the order of a few days (APT attack scenario).}
%     \label{fig:vary-alpha}
%     \vspace{-.5cm}
% \end{figure}
% Fig. \ref{fig:vary-alpha} (Top) shows a similar analysis, this time varying $\alpha$ in the range of 0 to 80m ($\smalltilde$5000s)  while using a constant $M$ of \$5,000. 
% We observe that when $\alpha$ is near 0, the cost  incurred by any malware is high immediately; hence, the static detector and the dynamic detector are both ``too slow'' and therefore have very expensive cost estimates.
% In fact, when using a very low $\alpha$ value, both detectors are more expensive than never alerting. 
% This is because for each true positive, both tools are taking on the (near maximum) cost incurred from the attack, but also the triage and IR costs, making the total more than the maximum attack cost incurred by never alerting.

% Fig. \ref{fig:vary-alpha} (Bottom) varies $\alpha$ between roughly 40 and 55m with $M = \$500,000$ (the worst-case, APT attack cost scenario). 
% This relatively uninteresting plot shows that the static detector beats the dynamic detector slightly, and that essentially cost is not varying in this range of $\alpha$ because attacks that are caught are detected long before this point. 

% Our overall conclusion is that static detector is superiorin both the normal and worst-case attack scenarios although if the malware takes a relatively long time to develop, the two tools are very similar in costs. 



==> beyond-the-hype-3 (2)/50-discussion.tex <==
%%% Takeaways Bobby rambled off that might fit: Overall results—you’ll get 35-55% detection w/ static detectors and maybe 60% w/ dynamic detectors (embarrassingly, scarily bad :dread emoji: ). Signature-based are still better overall b/c they are fast and have ~0 false positives. ML does indeed “generalize” tho—upping the ~3% detection rates of zerodays by the signature-based detectors to ~40%! In short you need both a signature-based detector and an ML based detector. Best combos are signature-based detection on your host (it can quarantine files preconviction), and a dynamic detector on the network (assuming SSL decryption in place to feed it). Dynamic detectors are…… SLOW. Have it automatically connect to all the hosts to quarantine of you can. The bright spots here:  false positives are very low  (like fractions of a percent false alert rate) and detection is fast. Lastly, 3 or more detectors working together doesn’t buy you much, but two does!

\section{Conclusions, Limitations, Next Steps, and Takeaways}
\label{sec:did-discussion}
This study describes experiments with four \hl{prominent} malware detection technologies aimed at helping an organization assess (Q1) the ML generalization hypothesis and (Q2) the added value of network-level malware detectors. 
Our results provide empirical quantification on the efficacy of four market-leading  malware detectors. 
The three ML tools demonstrated a minimal 2$\times $ increase in detection coverage for publicly available executables and a 10$\times $ increase in malware detection coverage for zero-day executables.  
Less intuitive perhaps was how well the host signature--based tool performed:  exhibiting the best (perfect) precision; demonstrating comparable recall ($\smalltilde$35\%) to the host ML--host tool; and, according to the cost model, performing the best overall \hl{for small percentages of hard (zero-day, polyglot, or APT-style) files and when maximum possible damage cost incurred by an undetected hard file was not much more than an $n-$day malware.
Notably, if one expects (1) more than a couple percent of malicious files to be zero-day, polyglot, or APT-style files, and (2)  the cost from an undetected hard file to be much greater than otherwise, ML-based detectors provide substantial savings; this provides a strong argument for pairing detectors.} 
Combining the signature-based tool with an ML-based tool enables malware detection ranges above 90\% for in-the-wild executables and above 60\% for zero-day malware. 
As demonstrated by increased recall and the new configuration of the cost model, substantial value is added by combining either of the two network-level tools to either host-level tool. Unsurprisingly, dynamic analysis incurs the cost of latency for increased recall, and both network-level detectors vary in their capabilities across protocols. 
Our results indicate that low false positive rates (precision $> $98\%) should be expected, with fast detection time for static detectors, but that this comes at the cost of recall. 
Of the four detectors in this study, none surpassed 55\% recall, and recall falls dramatically with JAR and polyglot file types.


Testing only four representative tools is a clear limitation; in particular, 
%inhibits the scope of the results to, e.g., we cannot make definitive statements about the state of current malware detection technologies as a whole.  
many COT tools offer (and some require) cloud connectivity to enhance detection at the expense of privacy, but no such tool was represented. 
Our test environment did not allow connection to the Internet, which might have stymied malware actions and therefore affected detection results. 
\hl{Similarly, network-level signature-based tools are not fully represented. }
Impact to host resources was not taken into account in this study (CPU, memory, and disk I/O, in particular). 
More sophisticated (and presumably more accurate) models of attack cost could be integrated in future work (e.g., \cite{Kondakci_2009}). 
Finally, accurate cost estimates from the cost model will require per-SOC inputs. Based on our parameter sensitivity analysis, the rankings and takeaways of the cost model results for these tools should generalize (and our treatment provides a blueprint for future use). 
%(especially for analyzing zero-days) without burdoning the host’s resources. This of course has a drawback of not being ``on-prem’’, that is, network data is sent to the vendor. No such tool was tested. 
% A rule of thumb quoted by SOC operators is that 80\% of traffic is encrypted. For our network-level file detectors, accurate file carving would in-practice rely on an SSL/TSL decrytion technology. We did not test tools with this added variable as our focus was on the file analyzers, yet understanding their effect is needed for true realism. 
% The complementary analysis (Sec. \ref{sec:tc2:heterosensinganalysis}) was performed with data analysis; As such it neglects the impact to host resources. Our assumptions for cost model inputs are reasonable for reasoning about these tools, but the model was used as a ranking/comparison tool, as opposed to seeking accurate cost estimates. This provides an example that can be tailored to each SOC’s specific inputs. 
Nevertheless, we argue that trends found among these four market leaders are sufficient to  pose hypotheses, raise awareness of gaps, and sharpen next-step research. 


% Perhaps the single greatest takeaway of this study is to prioritize next step research. 
We itemize priorities for next-step research from this work: 
% (1) Since malware detection is  first line of defense for nearly all personal and industrial computers, knowing how well/poor modern tools perform is worthwhile. 
% (1) A study with more breadth (more tools) and more depth (more samples) is warranted to quantify the state of the art in the wild (i.e., precision, recall, time-to-detect results per file type, per delivery protocol of COTS tools) with more significant evidence. 
% (2) Academic research produces a myriad of papers providing incremental gains in malware detection via applications of novel configurations of machine learning models. Indeed increased detection accuracy is needed 
Our polyglot detection results suggest that detectors are failing at preclassifying a file into possibly many file types for which it can execute. 
Research is needed to accurately and quickly determine \textit{all} of the file types of a given sample and integrate this capability into COTS detectors to enhance detection. 
Further research is needed to address the polyglot detection issue and performance with throughput and computational expense in mind. 
%is a well-formed and standard classification task at which standard applications of supervised ML (with domain expertise used to craft appropriate static features) should provide very accurate results. A viable file type detector that is robust to such trickery must also be prioritized. 
% Armed with this ability to know \textit{all} of the file types of a given sample, 
More accurate detection models for all file types are needed. 
In particular, future malware detection research should focus on increasing the detection capabilities for non-PE and non-MS Office file types. 
This might entail enhancing the quantity of malware and benignware files of many types that are currently less prevalent (e.g., through an effort to build and make public a more diverse malware data set). 
% As non-PE malware is harder to come by in such alternate file types, the research community may wish to put effort into compiling a more comprehensive set of such samples. 
For the two network-level detectors, recall varied widely when identical files were delivered on different protocols. 
%This suggest that the ability to carve files suffers across protocols but is a needed pre-step for network level detection. 
We suggest a study to identify whether the file carving is the limiting factor and to find methods for accurately extracting a copy of the file from the packet stream to the detector. 
\hl{Future work to tune the cost model to a specific SOC is both reasonable and likely very valuable if successful, especially if it produces a procedure and code-base for refitting to any SOC. 
Malware detection studies in which computational resources of the hosts are monitored and incorporated are needed, in particular for a higher fidelity cost model.  
As evidenced by our results, many of the takeaways depend on difficult assumptions; for example, the percent of files that are malware (e.g., Li et al. {\cite{li2017large}}) or the percent of different file types or categories in the wild. Empirical studies to provide data on cyber-related artifacts provides fodder for useful studies. }


Finally, some takeaways for SOCs. 
% Our results suggest that ML-based malware detectors will enhance and complement signature-based detection.  
% especially on PE files and zero-days, but none of the tools we tested are recommended as standalone defenses. 
Great gains in detection rate (recall) with few false positives (high precision) are permitted by all pairs of tools in our study, but little is gained from using more than two of these tools. 
When choosing a pair of tools, strive for tools that complement each other in terms of increasing the coverage (detection rate) of all file types, rather than duplicating results---this might require some preliminary testing with different file types. 
A feasibility study for any desired pairing of host tools is needed before deployment to examine how the combination will affect the host’s resources. 
Our results (Table \ref{tab:cost-add-to-host}) show that substantial savings are yielded by adding a network-level detector in all four combinations of network-to-host detectors tested.
% In our results, the dynamic detector yields by far larger gains than the static detector (3-14$\times$). 
The accuracy gains permitted by the dynamic detector in our study outweighed latency costs. 
For any network detector, testing bandwidth and file rates with the specific software and hardware is needed. 
Note that network-level detectors require unencrypted traffic, so we are presupposing that an SSL/TSL ``break and inspect'' technology is in place. 

% Overall, we hope that this study provides motivation for further research, worthwhile insights for SOCs looking to purchase tools, and a meaningful example of how to use the cost model proposed by Iannacone and Bridges~\cite{iannacone2020quantifiable}. 




% This real-world evaluation of malware detection tools focused on three core research questions: (1) Do ML-based malware detectors provide better detection than signature-based detectors?; (2) Is it worth purchasing a network-level malware detector to complement host-based detection?; and (3) What is the trade-off between detection time and detection accuracy among commercially available tools using static and dynamic analyses?
% In this section, we discuss the implications of our results for each of these key questions, the failure of tools to detect polyglot files or achieve high detection rates, and limitations.


% Many suspected results were attained and in-part quantified;  specifically, ML can indeed identify zero-days more effectively than signature-based detection, dynamic analysis is superior in recall to static but with a cost of detection latency, and resource allocation can prove critical for reasonable latency. 
% Regarding question (1), we found that the signature-based malware detection tool (host-based) exhibited the best (perfect) precision, comparable recall ($\smalltilde$35\%) to the host ML-host tool, and according to the cost model was the best overall balance of the two host-based tools. 
% Importantly, all ML-based tools performed far better at detecting malicious executables and zero-day malware. 
% \textbf{Indeed ML-based tools provide generalization capabilities to never-before-seen files, and could potentially replace signature-based tools, yet our results indicate that no tested detector is an adequate standalone malware defense. 
% }


% Regarding question (2), we first note that independent of this experiment, our experience with network-level malware detectors is that they do not in general block/prevent malware, while the host-based detectors generally provide pre-execution conviction and quarantine. Thus, using network-level tools as a standalone solution is not recommended. 
% In this experiment, we found that the detection efficacy of the network-level tools is dependent on the protocol being used (in addition to the filetypes that pose difficulties). 
% The HTTP protocol had the best overall results across the network-based technologies under test.  
% However, when network protocols other than HTTP and the Simple Mail Transfer Protocol (SMTP) were used, the detection results suffered. %for network-based detection were less compelling 
% See Table \ref{tab:detection-across-protocols}. 
% Future research on mature network-level malware detection technologies should focus on file carving capability and, specifically, on the reliability of the file carving across protocols.

% Regarding question (3), we found that the dynamic network-based detector is by far the best complement to ML- and host-based signature solutions because it detects categories of malware the other tools do not. See Tables \ref{tab:tc2:compl-analysis} \& \ref{tab:cost-add-to-host}.  
% However, dynamic malware analysis is significantly slower than static analysis (Figure \ref{fig:tc2:malware-analysis-times}). 
% We believe it is still a good decision to use the dynamic network-based detector in tandem with another solution, with the understanding that it will simply take longer to convict malicious files. 

% \subsection{Characterizing the State of the Art} 
% To our knowledge this is the first study of commercially available malware detection tools, and many important takeaways are uncovered. 
% \textbf{Our results indicate that the state of the art for this market is $34-55\%$ detection rates, with low false alerts (precision $>$96\%), and detection delays of under $\smalltilde 2$m for static tools. 
% Dynamic tools are significantly slower.} 
% Pairing detectors can achieve detection rates $\smalltilde 60\%$, but over 35\% of malware in our test is undetected! The single greatest takeaway of this report is that malware detection rates are surprisingly low. Future research to increase recall with little cost to precision and detection time is sorely needed. 


% Notably, all malware detection tools' ability to detect malware varies greatly per filetype, with the Host ML tools failing completely on non-PE files, and all tools nearly impotent on JARs and completely impotent on polyglots. 
% This result highlights two takeaways: (1) correct file type determination is critical to malware detection, and (2) uncertainty in file type determination is not communicated.
% % Research to develop ML models for accurate detection across many more filetypes is needed. 
% % We also found that the inclusion of polyglot files---those files with multiple valid file headers (see Section~\ref{rel:poly})---revealed a significant weakness across all evaluated malware detection technologies: a sensitivity to file type determination.  
% % In this case, file type refers to the format of the file and the nature of the data contained within the file, as captured in Table \ref{tab:tc2:comparative-analysis}.  
% % Despite strong overall malware detection performance with these tools, they all were completely stymied by the polyglot files.  
% %Based on these insights, one can infer the analytic process with respect to each of these technologies that starts with a file type determination, followed by an analytic process that is file type dependent.  
% % The polyglot files reveal a weakness in that process, where an inability to identify a file type seems to bypass any analysis.  
% %It is possible (but not confirmed) that many of these technologies use the same underlying libraries or commands to determine file type.
% There are ways to more accurately identify file type, but it is possible (though not confirmed) that many of these technologies choose to use less accurate libraries to maintain throughput. 
% More research is needed to help these tools accurately identify file type while maintaining acceptable throughput. 


% \subsection{Limitations of this study}
% Because we only consider complementary tools through data analysis, when considering the two host-level tools, the added impact to the host's resources are not taken into account. 

% Several limitations in our study can be addressed by future work. 
% As we selected one tool from each of the four malware detection methods,  future work could increase the number of tools from each category---or focus specifically on one of the chosen categories to verify that our findings generalize to tool types more broadly. 
% While a file corpus of over 3,500 samples is large in comparison to any prior work, it is not necessarily large in comparison to the amount of malware that exists in the wild. 
% % It is, therefore, difficult for us to determine whether or not our results have saturated.
% Future work should verify our results on additional malware samples and potentially expand this analysis using data from tools deployed in live SOC environments. 


% Our implementation of the cost model gives provides an attractive method to compare tools across many diverse
% attributes, while simulating actual costs for use. 
% In terms of actually producing an accurate dollar cost, many limitations of the model exist. Notably, no known data exists to estimate (a) the number of each file type expected to be seen by detector, nor (b) the  malware percentage of non-PE file types, nor (c) the average cost per malware, or better, per malware file type---let alone how that cost changes per time. 
% Future research to understand these distributions in the real world would greatly help such modeling efforts. 
% On the other hand, we showed that our model's rankings of the tools are robust with respect to varying inputs in reasonable ranges. In future work higher fidelity may result from varying the cost per file type (effectively weighting Zero-days more than $n$-day malware).  


% \section{Actionable Takeaways for Choosing Malware Detectors} 
% \label{sec:advice}
% Our cost model and statistical results show that if only one detector is possible, the Host Signature detector is the overall best. 



% Network-level tools are especially discouraged as standalone malware detectors for two reasons: (1) in our experience, they do not immediately quarantine detected files as host tools do (they detected, not prevented) and  (2) detection ability is very poor on some protocols. See Table \ref{tab:detection-across-protocols}.
% Using two tools is recommended, and our statistical results promote the Host 
% Signature detector paired with the Network Dynamic detector as the overall best---this pair boasts the highest detection rate and lowest number of false positives (highest recall and precision). See Table \ref{tab:tc2:compl-analysis}. 
% Detection efficacy varies greatly per file type (Tables \ref{tab:tc2:comparative-analysis} \& \ref{tab:tc2:compl-analysis}).
% Based on our results, ML-based detectors add the most value with respect to PE files. 
% Because all detectors demonstrated high precision (i.e., low FP rate) in our study, it makes sense to combine these sensing modes to achieve better detection rates. 

% We suspect many SOCs have a standard host-based detector, but are potentially interested in purchasing a network-level malware detector. 
% One can compare the estimated yearly costs of such a decrypter with the savings predicted in our Table \ref{tab:cost-add-to-host} if this is a required asset. 
% Finally, we recommend considering network-level detectors that provide native integration with already-deployed host-based software (e.g., host malware detector) for potential quarantine of network-detected files. 


%Another significant finding was the variation in detection performance based on network transport protocol.
%This variation applied to the two malware detectors that were network-based because their analysis process involved carving files out of network data streams for an off-host analysis.
%From an evaluation perspective, it does not appear to be an analytic issue, but rather an issue with the underlying libraries or commands that extract the files from the network data stream.  



%ML-based malware detectors also add significant detection coverage in analyzing JAR files, and are competitive with signature-based tools with respect to MS Office files and APT executables.  
%In particular with respect to signature-based and ML-based, it appears that combining these sensing modes is effective at increasing detection coverage. 
%A contributing factor to the complementary nature of signature-based and ML-based malware detectors is the high precision of all of the evaluated technologies.  
%The low false alert rate for all tools means there is minimal cost to a complementary sensing architecture.
 
%An argument could be made that AI/ML approaches to malware detection could replace signature-based approaches, as combinations of ML-based detectors competed with or exceeded signature-based detection rates, depending on file category.  
%However, detection times and similar additional factors make that distinction less clear.  Detection efficacy is more than an F1 Score.  Certainly there is massive process and infrastructure behind the event analysis and signature generation process that could represent a significant cost savings if eliminated.  However, a similarly rigorous process is necessary for the ML-based technologies, but with a focus on training data vetting and management.  Additionally, the APT category in this experiment, which was dominated by the signature-based tool, provided a good example of signatures detecting specific patterns well (in this case, those associated with a command/control framework), where the generalized approach of ML only partially detected.  These are evidences that support the results from this experiment that the combination of these different detection modes is the most effective approach. 

%Additionally, our evaluation of the strengths of the different malware detection technologies suggest that those tools that leverage ML to convict malware files have significantly better performance in detecting malicious executables.  
%ML tools  demonstrated (minimally) a 2x increase in detection coverage for publicly available executables and a 10x increase in malware detection coverage for zero day executables.  
%These are additive due to the high precision of both sensing modes, which enable malware detection ranges above 90\% for in-the-wild executables and above 60\% for zero day malware.  
%Combining malware detection technologies in this complementary way provides a powerful boost to detection efficacy. 
%Comparatively, ML-based malware detectors also add significant detection coverage in analyzing JAR files, and are competitive with signature-based tools with respect to MS Office files and APT executables.  
%However, the generalization performance of ML-based tools appears to add the most value with respect to executables. 

%Another key finding is that there is an overlap in detection coverage on the order of 80\% between pairs of ML-based tools.
%From a practical standpoint, this means that all three modes of ML-based sensing may not be necessary if sensor cost is a driver.
%The confirmatory analysis described in Section \ref{sec:tc2:heterosensinganalysis} helps to understand the overlap in malware detection coverage.  
%The complementary value of ML-based tools is evident based on the detection data, but it is unclear which or how many ML-based tools should be used to complement a signature-based baseline.  
%An overlap in detection capability reveals itself as the equivalency of the union and intersection of sensing combinations.  
%That is, if sensing combinations are combined in a complementary way, as in Table \ref{tab:tc2:compl-analysis} and their Precision and Recall values are equivalent, then there is an overlapping generalization performance.  









==> beyond-the-hype-3 (2)/90-acks.tex <==
\begin{acks}
% Acknowledgements redacted.
Thanks to Charlie Horak for the editorial review, and to the many reviewers whose constructive criticism helped polish this work. 

The research is based upon work supported by the Department of Defense (DOD), Naval Information Warfare Systems Command (NAVWAR), via the Department of Energy (DOE) under contract  DE-AC05-00OR22725. The views and conclusions contained herein are those of the authors and should not be interpreted as representing the official policies or endorsements, either expressed or implied, of the DOD, NAVWAR, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purposes notwithstanding any copyright annotation thereon. 
\end{acks}



